Chemical Reaction Dynamics under Vibrational Strong Coupling

In this thesis, we use classical, semi-classical and quantum-mechanical methods to simulate chemical reaction dynamics inside of an optical cavity. Within such a cavity, by selectively coupling vibrational modes of the reactants to the vacuum state of light, recent experiments have observed significant changes in reaction rates and equilibrium constants - all without any external input of energy. We investigate the dynamics of both a single reaction and an ensemble of N identical reactions coupled to the cavity. In our single reactant studies, we find significant modification to the rate of reaction and to its quantum-mechanical equilibrium constant. All of the effects observed in our single molecule studies are however found to diminish as the number of reactants is increased. For any experimentally relevant number of molecules, the cavity effects on the reaction rate and the equilibrium constant are therefore shown to be negligible within all theories considered in this thesis. This thesis therefore does not offer any explanation for the experimental observations. It does however highlight issues with all current theoretical work on this topic, and provides suggestions - in light of the results presented here and in recent literature - as to what might be required to explain these effects.

==> EXTRA/A1-OLD.tex <==
\chapter{\label{app:1-}Static Equilibrium Properties under VSC}
\minitoc


It was proven by Nitzan and friends that the static equilibrium properties of any classical system are unchanged by the presence of the Cavity. To understand why this is, let's define a 1D system with cavity polarization in this direction. The classical Hamiltonian (in mass-scaled coordinates) for this is;
\begin{equation}
\begin{split}
    H(p,q,P,Q) = H_s + H_c = \frac{p^2}{2} + V(q) + \frac{P^2}{2} + \frac{1}{2}\omega_c^2\left(Q - \frac{\epsilon}{\omega_c^2}\:\mu(q)\right)^2
\end{split}
\end{equation}
Here $\epsilon$ is the coupling constant between cavity and system. It can be expressed in terms of the  cavity frequency $\omega_c$, system volume $\Omega$ and permittivity constant $\epsilon_0$ as such; $\epsilon = \sqrt{\frac{\omega_c^2}{\Omega\:\epsilon_0}}$
The Cavity Born-Oppenheimer surface, $V_{CBO}$ can therefore be defined as the combined potentials;
\begin{equation}
    V_{CBO}(q,Q) =  V(q) + \frac{1}{2}\omega_c^2\left(Q - \frac{\epsilon}{\omega_c^2}\:\mu(q)\right)^2
\end{equation}
At equilibrium, the potential of the cavity and system will be minimized such that $Q = \frac{\epsilon}{\omega_c^2}\:\mu(q)$. This means that at equilibrium $V_{CBO}(q,Q)$ = $V(q)$ and therefore any equilibrium properties of the system will be unchanged by presence in a cavity. This beggs the question, what about in the quantum case? \newline \newline
\section{Integrating out the Cavity}
Let us `ring polymerize' $H(p,q,P,Q)$ to give  $H_n(\vc{p},\vc{q},\vc{P},\vc{Q})$ in which all variables have been transformed to vectors of length $n$, the index of which corresponding to the bead index. The Hamiltonian is as such;
\begin{equation}
\begin{split} 
    H_n(\vc{p},\vc{q},\vc{P},\vc{Q}) &= H_{s_n}(\vc{p},\vc{q}) + H_{c_n}(\vc{q},\vc{P},\vc{Q}) \\ \\
    \text{where} \:\:\:\:\: H_{s_n}(\vc{p},\vc{q}) &= T_{s_n}(\vc{p}) + V_{s_n}(\vc{q})\\
    &= \sum_{j=1}^{n} \frac{p_j^2}{2} + V(q_j) + \frac{1}{2}\omega_n^2(q_j -q_{j+1})^2  
    \\
    \\
    \text{and}\:\:\:\:\: H_{c_n}(\vc{q},\vc{P},\vc{Q}) &= T_{c_n}(\vc{P}) + V_{c_n}(\vc{q},\vc{Q}) 
    \\
    &=\sum_{j=1}^{n} \frac{P_j^2}{2} + 
    \frac{1}{2}\omega_c^2\left(Q_j - \frac{\epsilon}{\omega_c^2}\:\mu(q_j)\right)^2 +\frac{1}{2}\omega_n^2(Q_j -Q_{j+1})^2
\end{split}
\end{equation}
The ring polymer spring terms (those containing $\omega_n = \frac{1}{\beta_n\hbar}$ , where $\beta_n = \frac{\beta}{n}$) can be made diagonal by a normal mode transformation. This can be shown by writing out the cavity Hamiltonian in vector form and inserting the identity a couple times. Let us define $\vc{\mu}$ where $\mu_j = \mu(q_j)$, and $C =  \frac{\epsilon}{\omega_c^2}$. $\mt{K}$ is the matrix that generates the ring polymer spring terms. This matrix is identical to that of the H\"uckel matrix for an $n$ orbital cyclic system.
\begin{equation}
\begin{split} 
    H_{c_n}(\vc{q},\vc{P},\vc{Q}) &=  \sum_{j=1}^{n}\left( \frac{P_j^2}{2} + 
    \frac{1}{2}\omega_c^2\left(Q_j^2 - 2C\:\mu_j\:Q_j + C^2\:\mu_j^2\right) +\frac{1}{2}\omega_n^2(Q_j -Q_{j+1})^2 \right)\\
&\equiv  \frac{1}{2}\:\vc{P}^\top\vc{P} + 
    \frac{1}{2}\omega_c^2\left(\vc{Q}^\top\vc{Q} - 2C\vc{\mu}^\top\vc{Q} + C^2\vc{\mu}^\top\vc{\mu} \right) 
    +\frac{1}{2} \vc{Q}^\top\mt{K}\vc{Q}
\end{split}
\end{equation}
There exists (as seen in $2^{nd}$ year Physchem) a unitary matrix $\mt{U}$ that diagonalizes $\mt{K}$ such that $\mt{K} = \mt{U}\mt{\omega^2}\mt{U}^\top$ , a diagonal matrix of eigenvalues $\omega_k^2$. By inserting the identity, the Hamiltonian can be recast in the normal mode representation;
\begin{equation}
\begin{split} 
=  \frac{1}{2}\:\vc{P}^\top\mt{U}\mt{U}^\top\vc{P} + 
    \frac{1}{2}\omega_c^2&\left(\vc{Q}^\top\mt{U}\mt{U}^\top\vc{Q} - 2C\vc{\mu}^\top\mt{U}\mt{U}^\top\vc{Q} + C^2\vc{\mu}^\top\mt{U}\mt{U}^\top\vc{\mu} \right) 
    \\&\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:
    \:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:
    +\:\:\:\frac{1}{2} \vc{Q}^\top\mt{U}\mt{U}^\top\mt{K}\mt{U}\mt{U}^\top\vc{Q} \\
   \therefore \Tilde{H}_{c_n}(\vc{\Tilde{q}},\vc{\Tilde{P}},\vc{\Tilde{Q}})&=  \frac{1}{2}\:\vc{\tilde{P}}^\top\vc{\tilde{P}} 
   +
    \frac{1}{2}\omega_c^2\left(\vc{\tilde{Q}}^\top\vc{\tilde{Q}} - 2C\vc{\tilde{\mu}}^\top\vc{\tilde{Q}} + C^2\vc{\tilde{\mu}}^\top\vc{\tilde{\mu}} \right) 
    +\frac{1}{2} \vc{\tilde{Q}}^\top\mt{\omega^2}\vc{\tilde{Q}}\\
        \text{where }& \vc{\tilde{Q}} =\mt{U}^\top\vc{Q} \text{ and } \vc{\tilde{Q}}^\top =\mt{U} \vc{Q}^\top \text{  (analogous for other variables)}
\end{split}
\end{equation}
This Hamiltonian is now diagonal in these coordinates and therefore can be expressed as the sum of independent terms. This will allow Gaussian integrals to be done later.
\begin{equation}
   \tilde{H}_{c_n}(\vc{\Tilde{q}},\vc{\Tilde{P}},\vc{\Tilde{Q}})=  \sum_{k=1}^n\left(\frac{\tilde{P}_k^2}{2}+ 
    \frac{1}{2}\omega_c^2\left(\tilde{Q}_k - C\:\tilde{\mu}_k\right)^2
    +\frac{1}{2} \omega_k^2 \tilde{q}_k^2\right)
\label{eqn:Diagonal1dHam}
\end{equation}
Let us now consider some operator $\hat{O}(\hat{q})$. Nitzan has proven that $\left<O(q)\right>$, (classical hence no hat..) is independent of whether or not the Hamiltonian contains an optical cavity term. For a quantum system though lets see. Recall that for any $\hat{O}(\hat{q})$, in RPMD the value can be obtained via an average over all beads of the classical expectation value $\left<\hat{O}(\hat{q})\right> \simeq \frac{1}{n}\sum\limits_{j=1}^{n}\left< O(q_j)\right>$. 
\begin{equation}
    \left<\hat{O}(\hat{q})\right>_{C} \simeq \frac{\int d\vc{p} d\vc{q}\ d\vc{P} d\vc{Q}\: e^{-\beta_n H_n(\vc{p},\vc{q},\vc{P},\vc{Q})}\:\: \frac{1}{n}\sum\limits_{j=1}^{n} O(q_j)}
    {\int d\vc{p} d\vc{q}\ d\vc{P} d\vc{Q} \: e^{-\beta_n H_n(\vc{p},\vc{q},\vc{P},\vc{Q})}} 
\end{equation}
The subscript $C$ denotes that this is the degree of freedom within an optical cavity.
As $\vc{p}$ and $\vc{P}$ are separable degrees of freedom in $H_n(\vc{p},\vc{q},\vc{P},\vc{Q})$, these independent Gaussian integrals can be cancelled, giving;
\begin{equation}
    = \frac{\int d\vc{q}\ d\vc{Q}\: e^{-\beta_n (V_{s_n}(\vc{q})+V_{c_n}(\vc{q},\vc{Q}))}\:\: \frac{1}{n}\sum\limits_{j=1}^{n} O(q_j)}
    {\int  d\vc{q}\ d\vc{Q} \: e^{-\beta_n (V_{s_n}(\vc{q})+V_{c_n}(\vc{q},\vc{Q}))}} 
\label{eqn:expvalc}
\end{equation}
The observable outside of a cavity is analogously calculated as;
\begin{equation}
    \left<\hat{O}(\hat{q})\right>_0 \simeq  \frac{\int d\vc{q}\ \: e^{-\beta_n (V_{s_n}(\vc{q}))}\:\: \frac{1}{n}\sum\limits_{j=1}^{n} O(q_j)}
    {\int  d\vc{q}\ \: e^{-\beta_n (V_{s_n}(\vc{q}))} }
\label{eqn:expval0}
\end{equation}
Let us now define $g(\vc{q})$. This will be the integral of interest;
\begin{equation}
    g(\vc{q}) = \int d\vc{Q} e^{-\beta\:V_{c_n}(\vc{q},\vc{Q})}
\end{equation}
If $g$ is not a function of $q$, the observable inside of a cavity reduces to that found outside of a cavity. Lets find out. Firstly, the integral can be transformed into the normal mode coordinates, noting that the Jacobian of this orthogonal transformation will be $1$. In addition to this note the indexing of $k$ starting at zero. This is used throughout to allow clear modulo $n$ arithmetic as $q_n \equiv q_0$. This reflects the fact that $\omega_0$, the $0^{th}$ normal mode frequency, is zero;
\begin{equation}
\begin{split}
        g(\vc{q}) &= \int d\vc{Q} e^{-\beta_n\sum\limits_{j=1}^n \left(
        \frac{1}{2}\omega_c^2\left(Q_j - \frac{\epsilon}{\omega_c^2}\:\mu(q_j)\right)^2 +\frac{1}{2}\omega_n^2(Q_j -Q_{j+1})^2 \right)}
        \\
        &= \int d\vc{\Tilde{Q}} e^{-\beta_n\sum\limits_{k=0}^{n-1}\left(
    \frac{1}{2}\omega_c^2\left(\tilde{Q}_k - C\:\tilde{\mu}_k\right)^2
    +\frac{1}{2} \omega_k^2 \tilde{Q}_k^2\right)}
    \\
    &= \prod_{k=0}^{n-1}\int d\Tilde{Q}_k e^{-\frac{\beta_n}{2}\left( 
    \omega_c^2\left(\tilde{Q}_k - C\tilde{\mu}_k\right)^2
    + \omega_k^2 \tilde{Q}_k^2\right)}
\end{split}
\end{equation}
This integral can be solved by completing the square;
\begin{equation}
\begin{split}  
&= \prod_{k=0}^{n-1}\int d\Tilde{Q}_k e^{-\frac{\beta_n}{2(\omega_k^2 +\omega_c^2)}\left(\tilde{Q}_k - \frac{\omega_c^2 C \tilde{\mu}_k}{\omega_k^2 + \omega_c^2}\right)^2 
    - \frac{\beta_n C^2\tilde{\mu}^2\omega_c^2}{2}\left(\frac{\omega_c^2}{\omega_k^2 +\omega_c^2} -1\right) }
    \\
&= \prod_{k=0}^{n-1} e^{- \frac{\beta_n C^2\tilde{\mu}_k^2\omega_c^2}{2}\left(\frac{\omega_c^2}{\omega_k^2 +\omega_c^2} -1\right) }
\int d\Tilde{Q}_k \: e^{-\frac{\beta_n}{2(\omega_k^2 +\omega_c^2)}\left(\tilde{Q}_k - \frac{\omega_c^2 C \tilde{\mu}_k}{\omega_k^2 + \omega_c^2}\right)^2 }
\\
&= \prod_{k=0}^{n-1} 
\left(\frac{2(\omega_k^2 +\omega_c^2)}{\beta_n}\right)^{\frac{1}{2}}
e^{\frac{\beta_n C^2\tilde{\mu}_k^2\omega_c^2}{2}\left(\frac{\omega_k^2}{\omega_k^2 +\omega_c^2}\right) }
\\
&= 
e^{-\beta_n\sum\limits_{k=0}^{n-1} \left[ A_k-\frac{C^2\tilde{\mu}_k^2\omega_c^2}{2}\left(\frac{\omega_k^2}{\omega_k^2 +\omega_c^2}\right)\right] }
\end{split}
\end{equation}
where,
\begin{equation}
    A_k = -\frac{1}{2\beta_n}\ln\left(\frac{2(\omega_k^2 +\omega_c^2)}{\beta_n}\right) 
\end{equation}
% This can now be subbed back into \eqref{eqn:expvalc}, giving our final expression;
% \begin{equation}
%     \left<\hat{O}(\hat{q})\right>_{C} \simeq  
%     \prod_{k=0}^{n-1}  \frac{\int dq_k\: e^{- \frac{\beta_n C^2\tilde{\mu}_k^2\omega_c^2}{2}\left(\frac{\omega_c^2}{\omega_k^2 +\omega_c^2} -1\right)-\beta_n V_{s_n}(\vc{q})}\:\: \frac{1}{n}\sum\limits_{j=1}^{n} O(q_j)}
%     {\int dq_k  \: e^{  - \frac{\beta_n C^2\tilde{\mu}_k^2\omega_c^2}{2}\left(\frac{\omega_c^2}{\omega_k^2 +\omega_c^2} -1\right) - \beta_n V_{s_n}(\vc{q})}}
% \end{equation}
Re-combining the now integrated out bath with the system potential, an overall new potential $V_{sc_n}$ is formed
\begin{equation}
\begin{split}
    V_{sc_{n}} = \sum_{k=0}^{n-1}\left[ A_k - \frac{C^2\tilde{\mu}_k^2\omega_c^2}{2}\left(\frac{\omega_k^2}{\omega_k^2 +\omega_c^2}\right)\right]
    + \sum_{j=1}^{n}\left[V(q_j) + \frac{1}{2}\omega_n^2(q_j -q_{j+1})^2\right]  
\end{split}
\end{equation}
As $\omega_k = 0$ for $k=0$, the potential on centroid is independent
Now we need to re-align the coordinates. Let us transform back out of the normal mode coordinates of the cavity potential. 
% As an aside, for a classical system in a cavity ($1$-Bead Hamiltonian), $\omega_k^2 = 0$, meaning that;
% \begin{equation}
% \left<\hat{O}(\hat{q})\right>_{C_{n=1}} = \:\frac{\int dq\: e^{- \beta V_{s}(\vc{q})}\:O(q)}
%     {\int dq  \: e^{  - \beta V_{s}(q)}}
%     \equiv
% \left<\hat{O}(\hat{q})\right>_{0_{n=1}}
% \end{equation}
% This hence proves Nitzans arguement. For $n > 1$ however, this is not necessarily the case.
\begin{equation}
\begin{split}
\text{It is known that}\:\:\:& \omega_k = 2\omega_n \sin\left(\frac{k \pi}{n}\right)
\\
\text{let us define a}&\text{ diagonal matrix}\:\ \mt{\tilde{\eta}} \:\:,\text{where the $k$th diagonal entry, }\: \tilde{\eta}_k = 1-  \frac{\omega_c^2}{4\omega_n^2 \sin^2\left(\frac{k \pi}{n}\right) +\omega_c^2}  
\\
\text{Analogously}&\text{ to }\mt{K}\text{ , }\:\:\: \mt{\eta} = \mt{U}\mt{\tilde{\eta}}\:\mt{U}^\top
\\ \\
 \text{such that}\:   V_{sc_{n}} &= \sum_{k=0}^{n-1} \frac{ C^2\omega_c^2}{2}\: \tilde{\mu}_k^2\tilde{\eta}_k
    + \sum_{j=1}^{n}\left(V(q_j) + \frac{1}{2}\omega_n^2(q_j -q_{j+1})^2\right)
\\
&= \frac{C^2\omega_c^2}{2} \vc{\Tilde{\mu}}^\top\mt{\tilde{\eta}}\vc{\tilde{\mu}} + \sum_{j=1}^{n}\left(V(q_j) + \frac{1}{2}\omega_n^2(q_j -q_{j+1})^2\right)
\\
&= \frac{C^2\omega_c^2}{2} \vc{\Tilde{\mu}}^\top\mt{U}^\top\mt{U}\mt{\tilde{\eta}}\:\mt{U}^\top\mt{U}\vc{\tilde{\mu}} + \sum_{j=1}^{n}\left(V(q_j) + \frac{1}{2}\omega_n^2(q_j -q_{j+1})^2\right)
\\
&= \frac{C^2\omega_c^2}{2} \vc{\mu}^\top\mt{\eta}\vc{\mu} + \sum_{j=1}^{n}\left(V(q_j) + \frac{1}{2}\omega_n^2(q_j -q_{j+1})^2\right)
\\
&= \sum_{j=1}^{n}\left(\:V(q_j)  + \frac{1}{2}\omega_n^2(q_j -q_{j+1})^2 + \sum_{i=1}^n \frac{1}{2}\omega_c^2\eta_{ij}\:C^2 \mu_i\mu_j\right) 
\label{eqn:IntegratedOutCavityRPMD}
\end{split}
\end{equation}
% Its almost like now each bead in the ring polymer has it's own dipole. The overall force experienced by each bead will be, by Hamilton's equations, will be
% \begin{equation}
%     -\frac{\partial V_{SC_n}}{\partial q_j} = 
%     -\frac{\partial V(\vc{q})}{\partial q_j}    
%  + \sum_{i=1}^{n}\frac{1}{2}\omega_c^2\eta_{ij}\:C^2 \mu_i\frac{d\mu_j}{dq_j} + \frac{1}{2}\omega_n^2(q_j - 2q_{j+1})
% \end{equation}
% Recall that $\mt{\tilde{\eta}}$ is a positive definite matrix, as it's values, $\Tilde{\eta}_k \in \left[0, 1-\frac{\omega_c^2}{4\omega_n^2  +\omega_c^2}\right]$. Therefore $\mt{\eta}$, will also be positive definite (as the transformation is orthogonal). From the bounding of $\tilde{\eta}_k$, can an analytical expression for the bounding of $\eta_{ij}$ be calculated?\newline \newline If so this could imply the nature of interactions in \eqref{eqn:IntegratedOutCavityRPMD} giving some sort of physical intuition - using a ring-polymer based model - to the effects that a cavity has on a system.\newline \newline
% In addition to this, simulation SEP of a system within a cavity for a dipole linear in the system's coordinates can be done in normal mode representation, and using the Cayley propagator for both the ring polymer potential and the Cavity-Induced perturbations.
% \newline\
\section{Understanding $\mt{\eta}$}
The transformation matrix $\mt{U}$ and normal mode `dipole scalar' $\mt{\Tilde{\eta}}$ are defined as;
\begin{equation*}
    U_{jk} = 
    \begin{cases}
        \sqrt{\frac{1}{n}} & \text{ } k=0\\
        \sqrt{\frac{2}{n}} \cos(\frac{2\pi kj}{n}) & \text{ } 1 \geqslant k \geqslant \frac{n}{2}-1\\
        \sqrt{\frac{1}{n}}(-1)^j & \text{ } k = \frac{n}{2} \\
\sqrt{\frac{2}{n}} \sin(\frac{2\pi kj}{n}) & \text{ } \frac{n}{2}+1 \geqslant k \geqslant n-1
    \end{cases}
    \:\:\:\:\:\:\:\:\:\text{   and   }\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:
  \tilde{\eta}_k =  1- \frac{\omega_c^2}{4\omega_n^2 \sin^2\left(\frac{k \pi}{n}\right) +\omega_c^2} 
\end{equation*}
% Note the index of $k = 0 \rightarrow n-1$. This method of `python' indexing is used throughout.\newline \newline 
% The `dipole scalar' can therefore be transformed back into bead coordinates by a similarity transform as suggested in the introduction of $\mt{\Tilde{\eta}}$;
% \begin{equation}
% \begin{split}
%     \eta_{ij} &= \sum_{k=0}^{n-1} U_{ik}\: \Tilde{\eta}_{k} \:(U^\top)_{kj}
%     \\
%  &= \sum_{k=0}^{n-1} U_{ik}\: \Tilde{\eta}_{k} \: U_{jk}
%  \\
%   &= U_{i0}\: \Tilde{\eta}_{0} \: U_{j0} +
%   \sum_{a=1}^{\frac{n}{2}-1} U_{ia}\: \Tilde{\eta}_{a} \: U_{jk} +
%   \: U_{i\frac{n}{2}} \Tilde{\eta}_{\frac{n}{2}} \: U_{j\frac{n}{2}} +
%   \sum_{b=\frac{n}{2}+1}^{n-1} U_{ib}\: \Tilde{\eta}_{b} \: U_{jb}
%   \\& \\
%     \therefore\:\:\:\eta_{ij}&=  
%   \sum_{a=1}^{\frac{n}{2}-1} \frac{2}{n} \cos\left(\frac{2\pi a}{n}i\right)\cos\left(\frac{2\pi a}{n}j\right)\left(1-\frac{\omega_c^2}{4\omega_n^2 \sin^2\left(\frac{a \pi}{n}\right) +\omega_c^2}\right) \:\:
%  \\& \:\:\:\:\:\:\:\:
%   + \frac{1}{n}\left(1-\frac{\omega_c^2}{4\omega_n^2 +\omega_c^2}\right)(-1)^{i+j}\\ &
%   \:\:\:\:  \:\:\:\:\:\:\:\:\:\:\:\:\:\:
%  \:\:\: + \sum_{b=\frac{n}{2}+1}^{n-1} \: \frac{2}{n} \sin\left(\frac{2\pi b}{n}i\right)\sin\left(\frac{2\pi b}{n}j\right)\: \left(1-\frac{\omega_c^2}{4\omega_n^2 \sin^2\left(\frac{b \pi}{n}\right) +\omega_c^2}\right)
% \end{split}
% \end{equation}
% This expression gives $\mt{\eta}$ as a function of $\beta$, $n$ and $w_c$ only.Note that as $\Tilde{\eta} = 0$ the first term can be removed. If the limit of $n\rightarrow\infty$ gives $\mt{\eta} = \mt{0}$ then we will know for sure that static equilibrium properties cannot be captured by RPMD.
% \subsubsection{Diagonal terms}
% Looking back at the new potential in \eqref{eqn:IntegratedOutCavityRPMD} there seems to be a new effective dipole-self energy term for the $j^{th}$ bead; $\frac{1}{2}\omega_c^2\eta_{jj}\:C^2 \mu_j^2$. This is simply the Dipole Self Energy of the classical system, scaled by $\eta_{jj}$. As beads in the ring polymer are invariant to cyclic permutations, the `diagonal dipole scalar' (now abbreviated as $\mu_j$) \textit{may} also have the same properties.
% \begin{equation}
% \begin{split}
%     \eta_{j}&=  
%   \sum_{a=1}^{\frac{n}{2}-1} \frac{2}{n} \cos^2\left(\frac{2\pi a}{n}j\right) \Tilde{\eta}_a
%   + \frac{1}{n}(-1)^{2j}\Tilde{\eta}_{\frac{n}{2}}
%  + \sum_{b=\frac{n}{2}+1}^{n-1} \: \frac{2}{n} \sin^2\left(\frac{2\pi b}{n}j\right)\:\Tilde{\eta}_b
%  \end{split}
% \end{equation}
% As $\omega_k$ is an even function in the interval $k \in [0,\frac{n}{2}]$, $\tilde{\eta}_k$ will also be as such. This means that the terms in each sum can be paired together such that;
% \begin{equation}
% \begin{split}
%         \eta_{j}&=  
%   \sum_{a=1}^{\frac{n}{2}-1} \frac{2}{n} \left(\sin^2\left(\frac{2\pi b}{n}j\right) + \cos^2\left(\frac{2\pi a}{n}j\right)\right)\Tilde{\eta}_a
%   + \frac{1}{n}(-1)^{2j}\Tilde{\eta}_{\frac{n}{2}}
%   \\
%   &=  
%   \frac{1}{n}\sum_{a=0}^{n-1} \Tilde{\eta}_a
%   \\
% &=  
%   \frac{1}{n}\sum_{k=0}^{n-1} \left( 1 - \frac{\omega_c^2}{4\omega_n^2 \sin^2\left(\frac{k \pi}{n}\right) +\omega_c^2}\right)
% \\ \\
% \eta_{j}&=  
%   1 - \frac{1}{n}\sum_{k=0}^{n-1}\frac{\omega_c^2}{4\omega_n^2 \sin^2\left(\frac{k \pi}{n}\right) +\omega_c^2}
% \end{split}
% \end{equation}
% This still has the permutation symmetry of the ring polymer (phew!) and is non-zero provided there is more than one bead. The $n \rightarrow \infty$ limit of this what matters though. If this is $0$, the exact Quantum RPMD Hamiltonian will not have any extra `Dipole Self Energy' terms after all.
% \begin{equation}
% \begin{split}
%     \eta_{j_{E.Q.}} =   \lim_{n\to\infty} \left(1 - \frac{1}{n}\sum_{k=0}^{n-1}\frac{\omega_c^2}{4\omega_n^2 \sin^2\left(\frac{k \pi}{n}\right) +\omega_c^2}\right)
% \end{split}
% \end{equation}
% Recall that $\omega_n = \frac{1}{\beta_n\hbar} \equiv \frac{n}{\beta\hbar}$ so lets introduce $E_{C} = \frac{1}{2}\beta\hbar\omega_c $, the Zero Point Energy of the cavity in units of $k_BT$ such that;
% \begin{equation}
%         \eta_{j_{E.Q.}} =   \lim_{n\to\infty} \left(1 - \frac{1}{n}\sum_{k=0}^{n-1} \: \frac{E_C^2}{n^2\sin^2\left(\frac{k \pi}{n}\right) + E_C^2}\right)
% \end{equation}
% Using numerical methods this limit can be evaluated, giving $1$
% \subsubsection{Evaluation of the limit}
% The limit of $\eta_ij$ is quite a hefty one, but can be greatly simplified by first considering the limit of $\Tilde{\eta}_k$;
% \begin{equation}
% \begin{split}
% \Tilde{\2eta}_{k,\infty} = \lim_{n\to\infty} \left( 1- \frac{\omega_c^2}{\omega_k^2 +\omega_c^2}\right)
% \end{split}
% \end{equation}
% To solve this limit, the $n\to\infty$ of $\omega_k$ can firstly be considered;
% \begin{equation}
% \begin{split}
% \lim_{n\to\infty}(\omega_k) &= \lim_{n\to\infty} \left(2\omega_n \sin\left(\frac{k \pi}{n}\right)\right)
% \\
% &= \lim_{n\to\infty} \left(\frac{2n}{\beta\hbar} \sin\left(\frac{k \pi}{n}\right)\right)
% \\
% &= \frac{2}{\beta\hbar}\lim_{n\to\infty} \left(n \sum_{m=0}^{\infty}\frac{(-1)^m}{(2m+1)!}\left(\frac{k \pi}{n}\right)^{2m+1}\right)
% \\
% &= \frac{2}{\beta\hbar}\left(k\pi + \lim_{n\to\infty} \left(\sum_{m=1}^{\infty}\frac{(-1)^m}{(2m+1)!}\frac{(k \pi)^{2m+1}}{n^{2m}}\right)\right)
% \\
% \lim_{n\to\infty}(\omega_k) &= \frac{2k\pi}{\beta\hbar}
% \\&\\
% \therefore \:\:\:\: \Tilde{\eta}_{k,\infty} &= \frac{k^2\pi^2}{k^2\pi^2 + E_C^2}
% \end{split}
% \end{equation}
% This is true provided $k$ is finite. For $k$ close to $n$ however, the limit is not as such. The only way to solve the limit here is instead to define some finite number $k'$, some finite value such that  $k = n - k'$. The limit of $\omega_k$ for $k \lesssim n$ can now be done;
% \begin{equation}
% \begin{split}
%     \lim_{n\to\infty}(\omega_{k}) &= \lim_{n\to\infty} \left(\frac{2n}{\beta\hbar}\sin\left(\frac{(n-k') \pi}{n}\right)\right)
%     \\
%     &= \lim_{n\to\infty} \left(\frac{2n}{\beta\hbar}\left(
%     \sin\left(\pi\right) \cos\left(\frac{k' \pi}{n}\right)
%     -    \cos\left(\pi\right)    \sin\left(\frac{k'\pi}{n}\right)
%     \right)\right)
%     \\
%     &= \lim_{n\to\infty} \left(\frac{2n}{\beta\hbar} \sin\left(\frac{k' \pi}{n}\right)\right)
%     \\
% \lim_{n\to\infty}(\omega_k) &= \frac{2k'\pi}{\beta\hbar}
% \\&\\
% \therefore \:\:\:\: \Tilde{\eta}_{k\lesssim,n\to\infty} &= \frac{(n-k')^2\pi^2}{(n-k')^2\pi^2 + E_C^2}
% \end{split}
% \end{equation}


==> EXTRA/A1-StaticEqmProperties.tex <==
\chapter{\label{app:1-}Static Equilibrium Properties under VSC}
\minitoc
\section{Multidimensional Gneralisation}
Consider a molecular system. Assume it can be described by $m$ $3$-dimensional points, each of charge $c_i$ on a potential energy surface. If we write the entire system position operator as a vector, the dipole operator
\begin{equation}
    \hat \mu(\hat Q) = \left(\begin{matrix} \mu_x \\ \mu_y \\ \mu_z \end{matrix}\right)
     = \left(\begin{matrix} c_x^\top\hat Q \\ c_y^\top\hat Q \\ c_z^\top\hat Q \end{matrix}\right) \text{,}
\end{equation}
where
\begin{equation}
\begin{split}
    c_x^\top =& \left(\begin{matrix} c_1 & 0 & 0 & c_2 & 0 & 0 &...&c_m & 0 & 0\end{matrix}\right) \text{,}
\\
    c_y^\top =& \left(\begin{matrix} 0 & c_1 & 0 & 0 & c_2 & 0 &...&0 & c_m & 0\end{matrix}\right)\text{,}
\\
    c_z^\top =& \left(\begin{matrix} 0 & 0 & c_1 & 0 & 0 & c_2 &...&0 & 0 & c_m\end{matrix}\right)\text{.}
 \end{split}   
\end{equation}
The Hamiltonian of this system,
\begin{equation}
    \hat H(\hat P,\hat Q) = \frac{1}{2}\hat P^\top\hat P + \hat V(\hat Q) \text{.}
\end{equation}
At equilibrium, the potential energy of the entire system is minimized. This means that the position of each degree of freedom can be expanded about a global minima in potential $V(Q_0)$ such that,
\begin{equation}
    \hat H(\hat P,\hat Q) \simeq \frac{1}{2}\hat P^\top\hat P + \frac{1}{2}(\hat Q - Q_0)^\top V^{\prime\prime} (\hat Q - Q_0)+ \hat V(Q_0)
\end{equation}
where $V^{\prime\prime}$ is the Hessian of the system. By moving the origin to the coordinates $-Q_0$ and starting the zero of energy at $V(Q_0)$, the Hamiltonian of $m$ uncoupled  $3$-Dimensional harmonic oscillators of frequency $\omega_i$ is generated.
\begin{equation}
    \hat H(\hat P,\hat Q) = \frac{1}{2}\hat p^\top\hat p + q^\top U q \text{,}
\end{equation}
where
\begin{equation}
    (U)_{ij} = \delta_{ij} \omega^2_i \text{.}
\end{equation}
The dipole moment can also be transformed into normal modes,
\begin{equation}
\begin{split}
    \mu_x &= c^\top_x UU^\top\hat Q
    \\
    &=  \tilde c^\top_x \hat q \text{,}
\end{split}
\end{equation}
which is crucially still a linear function in the transformed molecular coordinates. For this reason, any system of charged particles at equilibrium can be approximated as a set of uncoupled harmonic oscillators, with a linear dipole function.
\section{N molecules}
Now let us consider $N$ of these molecular systems at equilibrium. In total there are now $n\times m = N$ degrees of freedom Let us assume that each system is independent, such that the total Hamiltonian inside of a cavity
\begin{equation}
    \hat{H}_{\rm tot} = \sum_{i=1}^n\left(\Hat{H}(\hat{p}_i,\hat{q}_i)\right) + \Hat{H}_{\rm cav}(\hat{p}_{\rm c},\hat{q}_{\rm c},\hat{\mu}_{\rm tot})\text{,}
\end{equation}
where 
\begin{equation}
    \hat{\mu}_{\rm tot} = \sum_{i=1}^n \hat \mu(\hat q_i)
\end{equation}
and 
\begin{equation}
    \Hat{H}_{\rm cav}(\hat{p}_{\rm c},\hat{q}_{\rm c},\hat{\mu}_{\rm tot}) = 
    \frac{\hat{p}_{\rm c}^2}{2} + 
\frac{1}{2}\omega_{\rm c}^2 \left(\hat{q}_{\rm c} + g \hat x \cdot\hat{\mu}_{\rm tot}\right)^2 \text{,}
\end{equation}
Where the unitless coupling constant $g = \frac{1}{\omega_c} \sqrt{\frac{\hbar}{2 \epsilon_0 V}}$.
The Hamiltonian of this system can be expressed in vector form,
\begin{equation}
    \hat{H}_{\rm tot} = \frac{1}{2}\vc{\hat q}^\top\mt{K}\vc{\hat q} + \frac{1}{2}\vc{\hat p}^\top\vc{\hat p} +  \frac{\hat{p}_{\rm c}^2}{2} + 
\frac{1}{2}\omega_{\rm c}^2 \left(\hat{q}_{\rm c} + g \tilde c^\top_x \sum_{i=1}^n  \hat q_i \right)^2 \text{,}
\end{equation}
where
\begin{equation}
    (\vc{\hat q})_i = \hat q_i \quad\text{,}\quad (\vc{\hat p})_i = \hat p_i
\end{equation}
and $\mt{K}$ diagonal matrix such that $(\mt{K})_{ij} = \delta_{ij}\:U $.
The coordinates can be transformed into the dark/bright modes of the system, such that $\{\hat q\} :\rightarrow\{\hat Q\}$ and analogous for $p$.
\begin{equation}
     \hat Q_k = \frac{1}{\sqrt{N}}\sum_{l=1}^N e^{\frac{2\pi \text{i}}{N}kl}\hat q_l \quad k=0,1,2\:...\:n-1
\end{equation}
the matrix $\mt{K}$ will remain unchanged as it is a diagonal matrix, giving
\begin{equation}
    \hat{H}_{\rm tot} = \frac{1}{2}\vc{\hat Q}^\top\mt{K}\vc{\hat Q} + \frac{1}{2}\vc{\hat P}^\top\vc{\hat P} +  \frac{\hat{p}_{\rm c}^2}{2} + 
\frac{1}{2}\omega_{\rm c}^2 \left(\hat{q}_{\rm c} + g \tilde c^\top_x \hat Q_0 \right)^2 \text{.}
\end{equation}
the Hamiltonian can now be written as
\begin{equation}
\hat{H}_{\rm tot} =\sum_{i=1}^{N-1}\left(\Hat{H}_{\rm mol}(\hat{P}_i,\hat{Q}_i)\right) + \Hat{H}_{\rm cav}(\hat{p}_{\rm c},\hat{q}_{\rm c},\hat{\mu}(\hat Q_0)) \text{.}
\end{equation}
The quantum partition function,
\begin{equation}
    Z = \int dq_c dQ_0...dQ_{N-1} \bra{q_c,Q_0...,Q_{N-1}}e^{-\beta\hat{H}_{\rm tot}}\ket{q_c,Q_0...,Q_{N-1}}
\end{equation}
can therefore be factorized into
\begin{equation}
    Z = \int dq_c dQ_0\bra{q_c,Q_0}e^{-\beta(\hat{H}_{\rm mol}(\hat{P}_0,\hat{Q}_0)+\hat{H}_{\rm cav}(\hat{p}_{\rm c},\hat{q}_{\rm c},\hat{\mu}(\hat Q_0))}\ket{q_c,Q_0} \times \prod_{i=1}^{N-1}Z_i \text{,}
\end{equation}
where
\begin{equation}
    Z_i = \int dQ_i \bra{Q_i}e^{-\beta\hat{H}_{\rm mol}(\hat P_i,\hat Q_i)}\ket{Q_i} \text{,}
\end{equation}
the partition function corresponding to a molecular \textbf{uncoupled} from an optical cavity. Hence at large $N$, the optical cavity will have no effect on the system's partition function.
\section{Integration of $g(\mathbf{q})$}
\begin{equation}
    g(\vc{q}) = \int\!d\vc{q_{\rm c}} e^{-\beta_n B} \text{,}
\label{eqn:g(q)}
\end{equation}
where
\begin{equation}
   B = \sum\limits_{j=1}^{n}\left(\frac{1}{2}\omega_{\rm c}^2(q_{\text{c}j} + C\mu(q_j))^2
+ \frac{1}{2}\omega_n^2(q_{\text{c}j} - q_{\text{c}j+1})^2 \right)\text{.}
\end{equation}
This integral can be done in the normal modes of the ring polymer. To achieve this let us write the exponent in vector form
\begin{equation}
\begin{split}
     B &= \sum\limits_{j=1}^{n}\left(\frac{1}{2}\omega_{\rm c}^2\left(q_{\text{c}j}^2 + C\mu(q_j)q_{\text{c}j} + C^2\mu(q_j)^2\right)
+ \frac{1}{2}\omega_n^2(q_{\text{c}j} - q_{\text{c}j+1})^2\right)
\\
&= \frac{1}{2}\omega_{\rm c}^2\left(\vc{q_{\rm c}}^{\top}\vc{q_{\rm c}} + C\vc{\mu}^\top\vc{q_{\rm c}} + C^2\vc{\mu}^\top\vc{\mu}\right)
+ \frac{1}{2}\vc{q_{\rm c}}^{\top}\mt{K}\vc{q_{\rm c}} \text{,}
\end{split}
\end{equation}
where
\begin{equation}
    (\vc{q})_j = q_j \quad \text{,}\quad     (\vc{q_{\rm c}}) = q_{\text{c}j} \quad \text{,}\quad      
    (\vc{\mu})_j = \mu(q_j) 
\end{equation}
and the ring polymer tridiagonal cyclic matrix
\begin{equation}
    (\mt{K})_{i,j} = (2\delta_{i,j} - \delta_{i,j+1} - \delta_{i+1,j} - \delta_{i,j-1} - \delta_{i-1,j})\omega_n^2
\end{equation}
There exists (as seen in $2^{nd}$ year Physchem H\"uckel) a unitary matrix $\mt{U}$ that diagonalizes $\mt{K}$ such that 
\begin{equation}
    \mt{K} = \mt{U}\mt{\omega^2}\mt{U}^\top \text{,}
\end{equation}
where $\mt{\omega^2}$ is diagonal matrix of eigenvalues $\omega_k^2$. By inserting the identity, $B$ can therefore be recast in the normal mode basis of the ring polymer.
\begin{equation}
\begin{split} 
B &= \frac{1}{2}\omega_{\rm c}^2\left(\vc{q_{\rm c}}^{\top}\mt{U}\mt{U}^\top\vc{q_{\rm c}} + C\vc{\mu}^\top\mt{U}\mt{U}^\top\vc{q_{\rm c}} + C^2\vc{\mu}^\top\mt{U}\mt{U}^\top\vc{\mu}\right)
+ \frac{1}{2}\vc{q_{\rm c}}^{\top}\mt{U}\mt{U}^\top\mt{K}\mt{U}\mt{U}^\top\vc{q_{\rm c}}
\\
&= \frac{1}{2}\omega_{\rm c}^2\left(\vc{\tilde{q}_{\rm c}}^{\top}\vc{\tilde{q}_{\rm c}} + C\vc{\tilde{\mu}}^\top\vc{\tilde{q}_{\rm c}} + C^2\vc{\tilde{\mu}}^\top\vc{\tilde{\mu}}\right)
+ \frac{1}{2}\vc{\tilde{q}_{\rm c}}^{\top}\mt{\omega^2}\vc{\tilde{q}_{\rm c}} \text{,}
\end{split}
\end{equation}
where
\begin{equation}
    \vc{\tilde{q}} =\mt{U}^\top\vc{q}\quad \text{ , }\quad \vc{\tilde{q}}^\top = \vc{q}^\top \mt{U}
\end{equation}
with the other variables defined analogously. 
\\
\indent
Let us now return to $g(\vc{q})$. As the normal modes transformation was unitary, the Jacobian of the transformation is 1, hence
\begin{equation}
\begin{split}
    g(\vc{q}) &= \int d\vc{\tilde{q}_{\rm c}} \:e^{-\beta B}
\\
    &= \prod_{k=0}^{n-1}\int d\Tilde{q}_{\text{c}k} \:e^{-\frac{\beta_n}{2}\left( 
    \omega_c^2\left(\tilde{q}_{\text{c}k} - C\tilde{\mu}_k\right)^2
    + \omega_k^2 \tilde{q}_{\text{c}k}^2\right)}
\end{split}
\end{equation}
This integral can now be solved by completing the square;
\begin{equation}
\begin{split}  
&= \prod_{k=0}^{n-1}\int d\tilde{q}_{\text{c}k}\: e^{-\frac{\beta_n}{2(\omega_k^2 +\omega_c^2)}\left(\tilde{q}_{\text{c}k} - \frac{\omega_c^2 C \tilde{\mu}_k}{\omega_k^2 + \omega_c^2}\right)^2 
    - \frac{\beta_n C^2\tilde{\mu}^2\omega_c^2}{2}\left(\frac{\omega_c^2}{\omega_k^2 +\omega_c^2} -1\right) }
    \\
&= \prod_{k=0}^{n-1} e^{- \frac{\beta_n C^2\tilde{\mu}_k^2\omega_c^2}{2}\left(\frac{\omega_c^2}{\omega_k^2 +\omega_c^2} -1\right) }
\int d\tilde{q}_{\text{c}k} \: e^{-\frac{\beta_n}{2(\omega_k^2 +\omega_c^2)}\left(\tilde{q}_{\text{c}k} - \frac{\omega_c^2 C \tilde{\mu}_k}{\omega_k^2 + \omega_c^2}\right)^2 }
\\
&= \prod_{k=0}^{n-1} 
\left(\frac{2\pi(\omega_k^2 +\omega_c^2)}{\beta_n}\right)^{\frac{1}{2}}
e^{\frac{\beta_n C^2\tilde{\mu}_k^2\omega_c^2}{2}\left(\frac{\omega_k^2}{\omega_k^2 +\omega_c^2}\right) }
\\
&= 
e^{-\beta_n\sum\limits_{k=0}^{n-1} \left[ A_k-\frac{C^2\tilde{\mu}_k^2\omega_c^2}{2}\left(\frac{\omega_k^2}{\omega_k^2 +\omega_c^2}\right)\right] } \text{.}
\end{split}
\end{equation}
where each normal mode has a constant `shift' independent of the coupling strength and coordinates,
\begin{equation}
    A_k = -\frac{1}{2\beta_n}\ln\left(\frac{2\pi(\omega_k^2 +\omega_c^2)}{\beta_n}\right) \text{.}
\end{equation}
The definition of the coupling constant can now be re-inserted to give our final expression
\begin{equation}
  g(\vc{q})  = 
e^{-\beta_n\sum\limits_{k=0}^{n-1} \left[ A_k-\frac{\hbar}{2 \epsilon_0 V}\tilde{\mu}_k^2
\left(\frac{\omega_k^2}{\omega_k^2 +\omega_c^2}\right)\right] } \text{.}
\end{equation}
% As $\omega_k = 0$ for $k=0$, the potential on centroid is independent
\section{Expansions of g}
Let us look at the exponent of~\eqref{eqn:g(q)}, removing $A_k$ (as this has no dependence on $C$ and therefore is just a constant energy `lamb' shift in the integrated out Hamiltonian), expanding it as a Taylor series,
\begin{equation}
\begin{split}
\sum_{k=0}^{n-1}\left[ \frac{C^2\beta_n\omega_c^2}{2} \left(\frac{\omega_k^2}{\omega_k^2 +\omega_c^2}\right)\tilde{\mu}_k^2
\right]
&\equiv \sum_{k=0}^{n-1}\left[ \frac{C^2\beta_n}{2} \omega_k^2\left(\frac{1}{1 + \omega_k^2/\omega_c^2}\right)\tilde{\mu}_k^2
\right]
\\
& =    \frac{C^2\beta_n}{2}\sum_{m=0}^{\infty} \sum_{k=0}^{n-1}\left[(-1)^m \frac{(\omega_k^2)^{m+1}}{(\omega_{\rm c}^2)^{m}}\tilde{\mu}_k^2
\right]
\\
&= \frac{C^2\beta_n}{2}\sum_{m=0}^{\infty} \left[\left(\frac{-1}{\omega_{\rm c}^2}\right)^m \vc{\tilde{\mu}}^\top (\mt{\omega^2})^{m+1} \vc{\tilde{\mu}} 
\right] \text{,}
\end{split}
\end{equation}
which we will now call $D$. In this form, the coordinates can be transformed back into the bead representation,
\begin{equation}
    D =  \frac{C^2\beta_n}{2}\sum_{m=0}^{\infty} \left[\left(\frac{-1}{\omega_{\rm c}^2}\right)^m \vc{\tilde{\mu}}^\top \mt{U}^\top\mt{U}(\mt{\omega^2}\mt{U}^\top\mt{U}...\:\mt{\omega^2})\mt{U}^\top\mt{U} \vc{\tilde{\mu}}
\right] \text{,}
\end{equation}
In this form we now have our old friend $\mt{K}$, the spring constant matrix,
\begin{equation}
\begin{split}
    D &=  \frac{C^2\beta_n}{2}\sum_{m=0}^{\infty} \left[\left(\frac{-1}{\omega_{\rm c}^2}\right)^m \vc{\mu}^\top(\mt{K})^{m+1}\vc{\mu}
\right]
\\
&=  \frac{\beta_n\hbar}{2\epsilon_0V\omega_c^2}\vc{\mu}^\top\mt{L}\vc{\mu} \text{,}
\end{split}
\end{equation}
where
\begin{equation}
\begin{split}
    \mt{L} &= \sum_{m=0}^{\infty} \left[\left(\frac{-1}{\omega_{\rm c}^2}\right)^m (\mt{K})^{m+1}
\right]
\end{split}
\end{equation}
This series only converges for $\omega_{\rm c} >> \omega_{\rm n}$ which is not true.
Another possible expansion would be,
\begin{equation}
\begin{split}
\sum_{k=0}^{n-1}\left[ \frac{C^2\beta_n\omega_c^2}{2} \left(\frac{\omega_k^2}{\omega_k^2 +\omega_c^2}\right)\tilde{\mu}_k^2
\right]
&\equiv \sum_{k=0}^{n-1}\left[ \frac{C^2\beta_n\omega_{\rm c}^2}{2} \left(\frac{1}{1 + \omega_c^2/\omega_k^2}\right)\tilde{\mu}_k^2
\right]
\\
& =    \frac{C^2\beta_n\omega_c^2}{2}\sum_{m=0}^{\infty} \sum_{k=0}^{n-1}\left[(-1)^m \frac{(\omega_c^2)^{m}}{(\omega_{\rm k}^2)^{m}}\tilde{\mu}_k^2
\right]
\\
&= \frac{C^2\beta_n\omega_c^2}{2}\sum_{m=0}^{\infty} \left[\left(-\omega_{\rm c}^2\right)^m \vc{\tilde{\mu}}^\top \left(\mt{\omega^{-2}}\right)^{m} \vc{\tilde{\mu}} 
\right] \text{,}
\end{split}
\end{equation}
where
\begin{equation}
    \mt{\omega^{-2}}\mt{\omega^{2}} = \mt{\mathcal{I}}
\end{equation}
The coordinates can now be transformed back;
\begin{equation}
\begin{split}
    &=  \frac{C^2\beta_n\omega_c^2}{2}\sum_{m=0}^{\infty} \left[\left(-\omega_{\rm c}^2\right)^m \vc{\tilde{\mu}}^\top \mt{U}^\top\mt{U}(\mt{\omega^{-2}}\mt{U}^\top\mt{U}...\:\mt{\omega^{-2}})\mt{U}^\top\mt{U} \vc{\tilde{\mu}}
\right] \text{,}
\\
&=  \frac{\beta_n\hbar}{2\epsilon_0V}\vc{\mu}^\top\mt{M}\vc{\mu} \text{,}
\end{split}
\end{equation}
where
\begin{equation}
\begin{split}
    \mt{M} &= \sum_{m=0}^{\infty} \left[\left(-\omega_{\rm c}^2\right)^m (\mt{K^{-1}})^{m}
\right]
\end{split}
\end{equation}
This series has the issue of needing to know the inverse of the spring constant matrix, so also isn't great.
\section{\label{app:K0proof}Proof of $K_0$ identity}
This quick proof allows the cavity-modified rate constant for reactions to be inferred from their outside-cavity values. Let us assume Eqn.~\eqref{eqn:KnpFinalExp} to be true
\begin{equation}
            K = \frac{\sum\limits_{r=0}^{N}{N \choose r}\:(N-r)\:K_0^{-r}\prod\limits_{i=1,2,3}\left[\frac{1}{\sinh(\beta\hbar\lambda_{ri}/2)}\right]}
    {\sum\limits_{r=0}^{N}{N \choose r}\:r\:K_0^{-r}\prod\limits_{i=1,2,3}\left[\frac{1}{\sinh(\beta\hbar\lambda_{ri}/2)}\right]} \text{. }
\end{equation}
If the coupling constants $g_{\rm A}$ and $g_{\rm B}$ are both $0$, then one would expect this expression to yield the uncoupled equilibrium constant $K_0$. Casting our attention to the Hessian from Eqn~\eqref{eqn:HessianBright} by which $\{\lambda_{r1},\lambda_{r2},\lambda_{r3}\}$ are obtained. As all terms containing $r$ are multiplied by either $g_{\rm A}$ or $g_{\rm B}$, when uncoupled, the eigenvalues will have no dependence $r$. This means the bright-state partition function may be factored out from each sum as a constant, allowing cancellation such that
\begin{equation}
            K_0 = \frac{\sum\limits_{r=0}^{N}{N \choose r}\:(N-r)\:K_0^{-r}}
    {\sum\limits_{r=0}^{N}{N \choose r}\:r\:K_0^{-r}}\text{. }
\label{eqn:KnPNOCAV}
\end{equation}
Looking at the denominator,
\begin{equation}
\begin{split}
    \sum\limits_{r=0}^{N}{N \choose r}\:r\:K_0^{-r} &= K_0^{-1}\sum\limits_{r=0}^{N}{N \choose r}\:r\:K_0^{-r+1}
    \\
    &= K_0^{-1}\sum\limits_{r=1}^{N}\frac{N!}{r!(N-r)!}\:r\:K_0^{-r+1}
    \\
    &= K_0^{-1}\sum\limits_{r=1}^{N}\frac{N!}{(r-1)!(N-(r-1))!}\:(N-(r-1))\:K_0^{-(r-1)} \text{.}
\end{split}
\end{equation}
Now let us introduce $r^\prime = r-1$, such that
\begin{equation}
\begin{split}
    \sum\limits_{r=0}^{N}{N \choose r}\:r\:K_0^{-r} &= K_0^{-1}\sum\limits_{r^\prime=0}^{N-1}\frac{N!}{(r^\prime)!(N-r^\prime)!}\:(N-r^\prime)\:K_0^{-r^\prime}
    \\
    &= K_0^{-1}\sum\limits_{r^\prime=0}^{N}\frac{N!}{(r^\prime)!(N-r^\prime)!}\:(N-r^\prime)\:K_0^{-r^\prime}
    \\
    &= K_0^{-1}\sum\limits_{r=0}^{N}{N\choose r}\:(N-r)\:K_0^{-r} \text{,}
\end{split}
\end{equation}
in which the prime was removed in the last step (as labelling was arbitrary). Inserting this back into Eqn.~\eqref{eqn:KnPNOCAV},
\begin{equation}
\begin{split}
    \frac{\sum\limits_{r=0}^{N}{N \choose r}\:(N-r)\:K_0^{-r}}
    {\sum\limits_{r=0}^{N}{N \choose r}\:r\:K_0^{-r}} &=      \frac{\sum\limits_{r=0}^{N}{N \choose r}\:(N-r)\:K_0^{-r}}
    {K_0^{-1}\sum\limits_{r=0}^{N}{N\choose r}\:(N-r)\:K_0^{-r}}
    \\
    &=K_0 \text{,}
\end{split}
\end{equation}
which confirms the prediction of \label{eqn:KnPNOCAV}, showing that the ratios of uncoupled single molecule partition functions is equal to the $N$-molecule equilibrium constant for a system uncoupled from an optical cavity.

==> EXTRA/A2-Kramer_sTheory.tex <==
\chapter{\label{app:2-}Kramer's Theory}
\minitoc

The underlying assumption of Transition State Theory is that there is no recrossing of the dividing surface. To this end, it can be shown to be the $t\rightarrow0^+$ limit of the rate constant,\cite{Hanggi1990} or the rate constant corresponding to maximum friction (corresponding to all trajectories starting at the dividing surface being so over-damped that no re-crossing is possible).
\newline\newline
TST theory is sufficient only to describe the short time limit of reaction rates. To fix this, add the changes via the time dependent transmission coefficient \cite{Lec2021};
\begin{equation}
    \kappa(t) = \frac{k(t) }{k(0^+)}
\end{equation}
A relatively simple expression for the transmission coefficient can be found in both the high and low friction limits of a simple $1$D transmission problem.\newline \newline
Kramer's Theory is used to approximate the dynamics at the top of the barrier using Diffusion  at the top. It relies on the steady-state approximation and thus will give the $t \rightarrow \infty$ limit of $\kappa$.\newline \newline 
Grote Hynes Theory is used to approximated dynamics such that the reaction occurs so fast the the other degrees of freedom are shown to be Non-Markovian and need to 'catch-up' with them. This is Non-Markovian dynamics and will be captured using a Generalized Langevin Equation.
\section{First Passage Times}
This equation will be used in the next two sections. The derivation of it  is gorgeous and comes from \cite{Zwan2001}.
\newline \newline\indent
Consider a set of variables $\textbf{a}$, governed by a Langevin equation. Let $\textbf{a}(t)$ and $p(\textbf{a},t)$ be the correspond to the position and distribution of position respectively of $\textbf{a}$ at time $t$. The initial position $\textbf{a}_0$ is in some 'volume' $V$ in $a$-space with a boundary $\partial V$. The initial condition for starting any strajectory at $\textbf{a}_0$ is as such;
\begin{equation}
    p(\textbf{a},0)=\delta(\textbf{a}-\textbf{a}_0) 
\end{equation}
The Fokker-Planck operator, $\mathscr{D}$ corresponding to the Langevin dynamics of the system is defined to evolve the probability distribution of $\textbf{a}$ in time such that;
\begin{equation}
    p(\textbf{a},t)=e^{t\mathscr{D}}p(\textbf{a},0)
\end{equation}
The probability of the particle remaining within the volume $V$ at time $t$ thus equals;
\begin{equation}
    S(t,\textbf{a}_0) = \int_{V}d\textbf{a}\:e^{t\mathscr{D}}\delta(\textbf{a}-\textbf{a}_0)
\end{equation}
Therefore the probability of transmission in some small time $dt$ at $t$ is;
\begin{equation}
\begin{split}
 S(t,a_0)-S(t+dt,a_0) &= \rho(t,\textbf{a}_0) dt
 \\
 \therefore \:\:\:
 \rho(t,\textbf{a}_0) &= -\frac{dS(t,\textbf{a}_0)}{dt}
\end{split}
\end{equation}
And the mean first passage time will be the integral of this probability distribution over all time;
\begin{equation}
    \tau(\textbf{a}_0) = \int_0^\infty dt\int_V d\textbf{a} \:e^{t\mathscr{D}}\delta(\textbf{a}-\textbf{a}_0)
\end{equation}
By inserting unity, and taking the adjoint, the integral can be made such that the operator is only operating on unity, thus allowing integration over $d\textbf{a}$. It should be remembered that $(e^{\hat{O}})^{\dagger} = e^{\hat{O^\dagger}}$ and that the adjoint of a real scalar is itself;
\begin{equation}
\begin{split}
\tau(\textbf{a}_0) &= \int_0^\infty dt\int_{-\infty}^{b}d\textbf{a} \:1\:e^{t\mathscr{D}}\delta(\textbf{a}-\textbf{a}_0)
\\
&= \int_0^\infty dt\int_{-\infty}^{b}d\textbf{a} \:\delta(\textbf{a}-\textbf{a}_0)\: e^{t\mathscr{D}^{\dagger}}\:1
\\
&= \int_0^\infty dt\: e^{t\mathscr{D}^{\dagger}}\:1
\end{split}
\end{equation}
Finally, pre-multiplication by $\mathscr{D}^{\dagger}$ allows mean first passage time to be determined by solving a simple inhomogeneous adjoint equation \cite{Zwan2001}
\begin{equation}
\begin{split}
\mathscr{D}^{\dagger}\tau(a_0) &= \mathscr{D}^{\dagger}\int_0^\infty dt\:e^{t\mathscr{D}^{\dagger}}\:1
\\
&= \int_0^\infty dt\frac{d}{dt}\:e^{t\mathscr{D}^{\dagger}}\:1
\\\ \therefore   \:\:\:
\mathscr{D}^{\dagger}\tau(\textbf{a}_0) =& -1 \:\:\: \text{with}\:\:\: \tau(\textbf{a})=0 \:\text{on}\: \partial v
\label{eqn:FRSTPSGTIME}
\end{split}
\end{equation}
\section{High-Friction Limit}
Consider a particle crossing a barrier in the presence of other degrees of freedom. In the high-friction limit, the problem can be seen as a first passage time calculation \cite{Zwan2001}. The particle will obey the Langevin Equation;
\begin{equation}
    \ddot{q} = -\gamma \Dot{q} - \frac{dV}{dq} + \sqrt{2\gamma k_BT}\eta
    \:\:\:\:\:\: \left<\eta (t)\eta(t')\right> = 2k_BT\gamma\delta(t-t')
\label{eqn:LE}
\end{equation}
In the \textbf{limit of overdamping} the particle's position will vary slowly, but momentum will be quick. For this reason, the evolution of the particle's phase-space distribution can be equivalently represented with the Fokker-Planck Equation corresponding to the $1$-Dimensional Smulochowski Equation. $D$ is the diffusion coefficient, which in this example is given by the Einstein-Smulochowski relation, $D=\frac{k_BT}{\gamma}$ As it will be useful in the next section, let us treat $D$.
\begin{equation}
\begin{split}
\frac{\partial p(q,t)}{\partial t} &=  \frac{\partial}{\partial q} D e^{-\beta V(q)} \frac{\partial}{\partial q} \left(e^{\beta V(q)} p(q,t)\right) 
\\ \therefore \:\:\:
\mathscr{D}&=  \frac{\partial}{\partial q}D e^{-\beta V(q)} \frac{\partial}{\partial q} e^{\beta V(q)}
\\ \therefore \:\:\:
\mathscr{D}^\dagger&= e^{\beta V(q)}\frac{\partial}{\partial q} e^{-\beta V(q)} D\frac{\partial}{\partial q}   
\label{eqn:SE}
\end{split}
\end{equation}
Using equation \eqref{eqn:FRSTPSGTIME}, the mean first passage time of any trajectory following the above Langevin Equations of Motion can be found;
\begin{equation}
\begin{split}
e^{\beta V(q_0)}\frac{\partial}{\partial q_0} e^{-\beta V(q_0)} D\frac{\partial}{\partial q_0} \: \tau(q_0) = -1
\end{split}
\end{equation}
Now, the boundary conditions. The definition of a reactant is such that $q_0\in(-\infty,q^\ddagger)$ which can be modelled as having an absorbative barrier at $q^\ddagger$ and a reflective barrier at $-\infty$, therefore the equation can be solved for $\tau(q_0)$ by integration, taking these limits into account\textbf{LOOK INTO LIMITS -> DIAGRAM?};
\begin{equation}
\begin{split}
 e^{-\beta V(q_0)} D\frac{\partial}{\partial q_0} \: \tau(q_0) &= -
\int_{-\infty}^{q_0} dq' e^{-\beta V(q')}
\\
\tau(q_0) &=  -\int^{q_0}_{q^\ddagger}dq \frac{e^{\beta V(q)}}{D}
\int_{-\infty}^{q} dq' e^{-\beta V(q')}
\\
&=  \int_{q_0}^{q^\ddagger}dq \frac{e^{\beta V(q)}}{D}
\int_{-\infty}^{q} dq' e^{-\beta V(q')}
\label{eqn:IntSE}
\end{split}
\end{equation}
Now to deal with these integrals. By taking a locally harmonic approximation of the potential at the reactants; $V_R(q) \approx  \frac{1}{2}\omega_{r}^{2}(q-q_r)^2$, and at the dividing surface; $V_\ddagger(q) \approx  E_0^\ddagger - \frac{1}{2}\omega_{b}^{2}(q-q^\ddagger)^2$;
\begin{equation}
\begin{split}
\int_{q_0}^{q^\ddagger}dq e^{\beta V(q)}
\int_{-\infty}^{q} dq' e^{-\beta V(q')}
    \approx 
    \int_{q_0}^{q^\ddagger} dq 
    e^{\beta \left(E_0^\ddagger - \frac{1}{2}\omega_{b}^{2}(q-q^\ddagger)^2\right)} 
    \int_{-\infty}^{q}dq' 
     e^{-\beta \left(\frac{1}{2}\omega_{r}^{2}(q'-q_r)^2 \right)}
\end{split}   
\end{equation}
This approximation is justified as each integral is dominated by the contribution centered at the Taylor Expansion as done. \newline
\indent For the left hand integral, the largest contribution to the integral is when $q \rightarrow q^\ddagger$, therefore this lower limit can be extended to $-\infty$ such that the integral is half of a Gaussian centered at $0$\newline
\indent For the right hand integral, the largest contribution to the integral is when $q \rightarrow q_0$. So, provided $q^\ddagger > q_0$ such that there is minimal overlap between Gaussian double integrals, the upper limit can be extended to $\infty$. \textbf{DIAGRAM NEEDED}
\begin{equation}
\begin{split}
    \int_{q_0}^{q^\ddagger} dq& 
    e^{\beta \left(E_0^\ddagger - \frac{1}{2}\omega_{b}^{2}(q-q^\ddagger)^2\right)}
    \int_{-\infty}^{q}dq' 
     e^{-\beta \left(\frac{1}{2}\omega_{r}^{2}(q'-q_r)^2 \right)}
       \\ &\approx 
    \frac{1}{2}\int_{-\infty}^{\infty} dq 
    e^{\beta \left(E_0^\ddagger - \frac{1}{2}\omega_{b}^{2}(q-q^\ddagger)^2\right)} 
    \int_{-\infty}^{\infty}dq' 
     e^{-\beta \left(\frac{1}{2}\omega_{r}^{2}(q'-q_r)^2 \right)}
\\ 
&= \frac{1}{2}  \:
    \sqrt{\frac{2\pi}{\beta\omega_b^2}}\:e^{\beta E_0^\ddagger}\:\sqrt{\frac{2\pi}{\beta\omega_r^2}}
\\ \\
\therefore\:\:  & \tau \approx \frac{1}{2D}\frac{2\pi k_BT}{\omega_r\omega_b}e^{\beta E_0^\ddagger}
\end{split}
\end{equation}
The rate of arrival to the barrier is $1/\tau$. Note that the  As the arrival can be in either directions, the rate of crossing (in one direction) must equal half of this. Therefore, after inserting the Einstein relation;
\begin{equation}
    k_{SD} = \frac{\omega_b \omega_r}{2\pi\gamma} e^{-\beta E_0^\ddagger}
\end{equation}
By recalling that $\nu_b = \frac{\omega_b}{2\pi} = \frac{k_BT}{h}$ (as used in the derivation of the Eyring Equation), in this high friction or \textbf{spatial diffusion limit} the result is proportional to TST, corresponding to a transmission coefficient as;
\begin{equation}
    \kappa_{SD} = \frac{\omega_b}{\gamma}
\end{equation}
In this limit, the transmission coefficient is dominated by the motion over the barrier, hence the reciprocal dependence on the solvent friction. 
\section{Low-Friction Limit}
 In the low-friction limit, barrier crossing is frequent, with energy being lost to the surroundings slowly. Once a trajectory has lost enough energy to be confined to a single well, it can be said that the reaction has occured. Thus the rate of relaxation to equilibrium can be said to be controlled by the rate of energy diffusion; hence the \textbf{energy diffusion limit} is this place. The derivation for these dynamics has been copied from \cite{Zwan2001} and starts with the Fokker-Plank equation for the phase space distribution function $f(q,p;t)$ corresponding to the Langevin Equation given in \eqref{eqn:LE}
 \begin{equation}
     \frac{\partial }{\partial t}f(p,q;t) = -L_0 f + \gamma k_BT 
     \frac{\partial}{\partial p} f_{eq}
     \frac{\partial}{\partial p} \frac{f}{f_{eq}}
\label{eqn:FP}
 \end{equation}
 where $L_0$ is the Classical Liouville operator just as in \eqref{eqn:LiouCl} and $f_{eq}$ is the equilibrium distribution, given by the unpeturbed Hamiltonian; $H=\frac{p^2}{2m}+V(q)$\newline\indent
 To transform this distribution into Energy coordinates, integration over distribution for all constant values of energy can be done
\newline \newline
The transform is as follows. As energy is conserved for an unpeterbed system, $L_0H=0$
\begin{equation}
\begin{split}
\frac{\partial}{\partial t} g(E;t) &= \int dpdq\:\delta(H-E)\:\frac{\partial}{\partial t} f(q,p;t) 
\\
&= \gamma k_BT \int dpdq\:\delta(H-E)\:\frac{\partial}{\partial p} f_{eq}
     \frac{\partial}{\partial p} \frac{f}{f_{eq}}
\label{eqn:FPT}
\end{split}
\end{equation}
The assumption now comes here. As the position and momenta are varying on a much faster timescale than the total energy of each trajectory in this energy diffusion limit, the distribution function of the particle can be approximated  as some function of the Hamiltonian; $f(q,p;t) \rightarrow \phi(H;t)$ and $f_{eq}(q,p) \rightarrow \phi_{eq}(H)$. This function has the constraint such that it leads to the correct energy distribution;
\begin{equation}
\begin{split}
 g(E;t)&=\int dpdq \delta(H-E)\Phi(H;t)
 \\
 &=\Phi(E;t)\int dpdq \delta(H-E)
 \\
\therefore\:\: \phi(E;t) = \frac{g(E;t)}{\Omega(E)} \:\:\: &\text{and likewise, } \:\:\:
\phi_{eq}(E) = \frac{g_{eq}(E)}{\Omega(E)}
\end{split}
\end{equation}
Where $\Omega(E)$ is the microcanonical partition function. So by insertion of this new definition and application of the chain rule;
\begin{equation}
    \phi_{eq}(E)\frac{\partial}{\partial p} \frac{f(q,p;t)}{f_{eq}(x,p)} 
    \approx 
    \frac{g_{eq}(E)}{\Omega(E)} \frac{p}{m}\frac{\partial}{\partial H}\frac{g(H;t)}{g_{eq}(H)}
\label{eqn:aprox2}
\end{equation}
 Insertion of \eqref{eqn:aprox2} into \eqref{eqn:FPT} and following integration by parts over momentum and observing $\frac{\partial}{\partial p}=\frac{\partial}{\partial E}\frac{p}{m}$, allows \eqref{eqn:FPT} to be written in "Smulochowski" form \cite{Zwan2001} with almost the exact same form as \eqref{eqn:SE};
 \begin{equation}
 \frac{\partial g(E;t)}{\partial t} \approx 
 \frac{\partial}{\partial E} 
D(E)g_{eq}(E)
 \frac{\partial}{\partial E} \frac{g(E;t)}{g_{eq}(E)}
 \end{equation}
 where,
 \begin{equation}
\begin{split}
D(E) = \gamma k_BT \frac{\int dpdq \left(\frac{p}{m}\right)^2 \delta(H-E)}{\Omega(E)}
\end{split}
 \end{equation}
 $D(E)$ is the Energy Diffusion constant. By noticing that $\delta(H-E) \equiv \delta(p^2 - 2m(E-V(q)))$, and thus integrating the numerator over $dp$ yields;
 \begin{equation}
D(E) =  \frac{\gamma k_BT}{m} \frac{\int dq \sqrt{2m(E-V(q))}}
{\Omega(E)}
 \end{equation}
 \textbf{ASK ABOUT SQUARE BRACKETS FOR FUNCTIONALS}\newline
 The integral is over all $q$ such that $E>V(q)$, which in fact corresponds to (half) of the integral of $p(q)$ around a complete cycle of $q$. This is the action; $I(E)$ \cite{Zwan2001} \newline \newline
 *Finally* , we can write down $\tau(E)$, just as in \eqref{eqn:IntSE}, as
 \begin{equation}
     \tau(E_0)=  \int_{E_0}^{E^\ddagger_0}dE \frac{1}{g_{eq}(E)D(E)}
\int_{0}^{E} dE' g_{eq}(E')
 \end{equation}
 Substituting the expressions for $g_{eq}$ and $D(E)$ yields,
 \begin{equation}
     \tau(E_0) = \frac{2m}{\gamma k_BT}
     \int_{E_0}^{E^\ddagger_0}dE
     \frac{e^{\beta E}}{I(E)}
\int_{0}^{E} dE' 
\Omega(E')e^{-\beta E'}
\label{eqn:tauintegral}
 \end{equation}
 At low temperatures, the Mean First Passage Time can be approximated from \eqref{eqn:tauintegral} as;
 \begin{equation}
\begin{split}
 \tau &\approx \frac{2\pi m k_BT}{\gamma}\frac{1}{\omega_r I(E_0^\ddagger)}e^{\beta E_0^\ddagger}
 \\
 \therefore \:\:\: k_{ED} &\approx \frac{\gamma \omega_r I(E_0^\ddagger)}{4\pi m k_BT} e^{-\beta E_0^\ddagger}
 \\
  \therefore \:\:\: \kappa_{ED} &\approx \frac{\gamma \omega_r I(E_0^\ddagger)}{2 m \omega_bk_BT} 
\end{split}
 \end{equation}
 As shown above, $\kappa_{ED} \sim \gamma$ showing that a completely different friction - reaction rate dependence than for high friction.
 \section{Putting these limits together}
 As shown in these previous sections, $\kappa_{SD}\sim\ \frac{1}{\gamma}$ and $\kappa_{ED}\sim\gamma$. By using Kramer's Interpolation Formula \cite{Kramers1940} these limits can be interpolated to show Kramer's Turnover.
 \begin{equation}
     \frac{1}{\kappa} = \frac{1}{\kappa_{SD}} + \frac{1}{\kappa_{ED}}
 \end{equation}
 When these limits 
%  \begin{figure}[H]
% \centering
% % \includegraphics{text/Tools/Fig1.png}
% \caption{Connection of the Spacial and Energy Diffusion limits}
% \label{fig:fig1}
% \end{figure}
As shown in \(\ref{fig:fig1}\) There is some optimum friction where the rate of reaction is maximized. Throughout this thesis there will be graphs that look very similiar to this, and the explanations will follow the same logic. \newline\newline
In this section for dynamical corrections, it was assumed that the friction experienced by any trajectory $\gamma$, was a constant in the equations of motion (see \eqref{eqn:LE} for example). This of course is not true.

==> EXTRA/EqmResults.tex <==
Firstly let us consider single-molecule effects - scanning against $\omega_{\rm c}$ to find values of $\Delta\omega$ and $\rho$ that maximise cavity effects on equilibrium constants. The light-matter coupling constant is fixed at its maximum value from Sec.~\ref{3:PR} such that $\eta_{\rm c} = {5\times10^{-3}}{\rm au}$.
\begin{figure}
\centering
\begin{subfigure}[c]{0.485\textwidth}
  \centering
\scalebox{1.}{\includegraphics[width=\textwidth]{figures/5.4-dwScan}}
\end{subfigure}
\hfill
\vrule
\begin{subfigure}[c]{0.485\textwidth}
  \centering
  \scalebox{1.}{\includegraphics[width=\textwidth]{figures/5.4-rhoScan}}
\end{subfigure}
\caption[Equilibrium properties parameter scan]{A scan over frequency miss-match (left panel) and polarity imbalance (right panel) to find conditions under which the optical cavity most affects the ratio of cavity-coupled to uncoupled equilibrium constants $K/K_0$ for a \textbf{single molecule reaction}. }
\label{fig:EqmPScan}
\end{figure}
Just as for transition state theory, Fig.~\ref{fig:EqmPScan} shows no focused `resonance' effects, but instead effects are observed over a broad range of $\omega_{\rm c}$. This could imply that, if the Hamiltonian used is sufficient in descriptions of polaritons, higher order cavity modes - which would be far away from resonance and therefore would not be observed in the infrared spectrum - could still have a sizable effect on equilibrium constants. This observation does raise the question of whether the common neglection of non-resonant cavity modes is responsible for the lack of theoretical understanding of the effects.
\\
\indent
Both equilibrium constant enhancement and suppression are observed, the trend of which is reversed when the well height imbalance, $E_{\rm A} - E_{\rm B}$, is reversed. For these plots, we have fixed $\rho = 0.5$ for left panel (as this was found to give least effect for any given $\Delta\omega$) and $\Delta\omega = 0$ for right panel (analogous for any given $\rho$). Now by selecting parameters that maximise the single molecule effect, let us see whether effects survive in the collective regime. As always, we will keep $\eta_{c}\sqrt{N}$ constant, such that the Rabi splitting is constant as $N$ increases.
\begin{figure}[!h]
\centering
\includegraphics[trim={0.25cm 0.25cm 0.cm 0.25cm}]
{figures/5.4-EqmColeff}
\caption[Equilibrium effects in the collective regime]{Any equilibrium effects observed `scale out' as $N$ is increased. The lines are chosen to illustrate that this effect is experienced throughout the (very large) parameter space}
\label{fig:eqmColeff}
\end{figure}
\FloatBarrier
\indent 
Fig.~\ref{fig:eqmColeff} shows the same `scaling-out' behaviour as previously observed in Fig.~\ref{fig:ResNP}. Note that in preliminary tests very many possible values of $\Delta\omega$, $\omega_{\rm c}$ and $\rho$ were tested - all with analogous results. This concludes our examination of polariton chemistry. Next chapter we will summarise our findings, discussing the possible insights this thesis had given towards the understanding of chemistry under vibrational strong coupling.

==> EXTRA/OLDproof.tex <==
In this section we will discuss the effect of an optical cavity on the partition function of a quantum system.
Let us reconsider the Pauli--Fierz Hamiltonian of Eqn.~\eqref{eqn:PF}, as earlier mentioned in section \ref{3:PFHam},
\begin{equation}
\Hat{H}_{\rm cav} =  \frac{\hat{p}_{\rm c}^2}{2} + 
\frac{1}{2}\omega_{\rm c}^2 \left(\hat{q}_{\rm c} + \sqrt{\frac{2}{\omega_{\rm c}}}\eta_{\rm c}\cdot\hat{\mu}\right)^2  \text{,}
\end{equation}
The interaction between cavity and system - with system dipole in the direction of field polarization - can therefore be extracted as
\begin{equation}
    \hat{V}_{\rm cav}(\hat{q},\hat{q}_c) = \frac{1}{2}\omega_{\rm c}^2(\hat{q}_{\rm c} + C\hat{\mu}(\hat{q}))^2\text{,}
\end{equation}
where we have defined a coupling constant, $C= \frac{1}{\omega_{\rm c}}\sqrt{\frac{\hbar}{\epsilon_0 V}}$. The constants used are the same as in Sec.~\ref{3:PFHam}. For a system inside of an optical cavity, using mass-scaled coordinates, the total potential energy,
\begin{equation}
    \hat{V}_{\rm tot.}(\hat{q},\hat{q}_{\rm c}) = \hat{V}_{\rm mol}(\hat{q}) + \hat{V}_{\rm cav}(\hat{q},\hat{q}_{\rm c}) \text{,}
\end{equation}
and the total kinetic energy,
\begin{equation}
    \hat{T}_{\rm tot.}(\hat{p},\hat{p}_{\rm c}) = \frac{\hat{p}^2}{2} +  \frac{\hat{p}_c^2}{2} \text{.}
\end{equation}
The system outside of the cavity can also be described with the same Hamiltonian - simply by setting the coupling strength $C = 0$. The `ring polymerized' form of the total Hamiltonian, found by following the method of Fig~\ref{fig:D-RPMD} is therefore
\begin{equation}
\begin{split}
& \quad\quad\quad\quad
\hat{H}_{\rm tot}(\hat{p},\hat{q},\hat{p}_{\rm c},\hat{q}_{\rm c}) \simeq H_{n}(\vc{p},\vc{q},\vc{p_{\rm c}},\vc{q_{\rm c}})
 \\
 = \sum_{j=1}^{n} &\left(T_{\rm tot}(p_j,p_{\text{c}j}) + V_{\rm tot}(q_j,q_{\text{c}j})
+ \frac{1}{2}\omega_n^2(q_j - q_{j+1})^2 
+ \frac{1}{2}\omega_n^2(q_{\text{c}j} - q_{\text{c}j+1})^2 \right)
 \text{.}
\end{split}
\end{equation}
The partition function of this system is therefore
\begin{equation}
    Q = \left(\frac{1}{2\pi\hbar}\right)^{2n}\!\int\!d\vc{p}d\vc{q}d\vc{p_{\rm c}}d\vc{q_{\rm c}} \:e^{-\beta_n H_{n}(\vc{p},\vc{q},\vc{p_{\rm c}},\vc{q_{\rm c}})} \text{.}
\end{equation}
As this is now a classical partition function, in which all terms therefore commute, integration over all momenta can be done to give
\begin{equation}
\begin{split}
   Q = \left(\frac{1}{\hbar}\right)^{2n}\!\int\!d\vc{q} \: g(\vc{q}) e^{-\beta_n \sum\limits_{j=1}^{n}\left(V_{\rm mol}(q_j)
+ \frac{1}{2}\omega_n^2(q_j - q_{j+1})^2 \right)} \text{,}
\label{eqn:Q-int.out.mom.}
\end{split}
\end{equation}
where
\begin{equation}
    g(\vc{q}) = \int\!d\vc{q_{\rm c}} e^{-\beta_n \sum\limits_{j=1}^{n}\left(V_{\rm cav}(q_j,q_{\text{c}j})
+ \frac{1}{2}\omega_n^2(q_{\text{c}j} - q_{\text{c}j+1})^2 \right)} \text{.}
\label{eqn:g(q)}
\end{equation}
The integration of $g(\vc{q})$ is done in appendix~\ref{app:1-} to yield
\begin{equation}
   g(\vc{q}) = \prod_{k=0}^{n-1} 
\left(\frac{2\pi(\omega_k^2 +\omega_c^2)}{\beta_n}\right)^{\frac{1}{2}}
e^{\frac{\beta_n C^2\tilde{\mu}_k^2\omega_c^2}{2}\left(\frac{\omega_k^2}{\omega_k^2 +\omega_c^2}\right) } \text{,}
\end{equation}
where $\omega_k = 2\omega_n \sin\left(\frac{k \pi}{n}\right)$, the ring polymer normal mode frequencies, and 
\begin{equation}
    \tilde{\mu}_k = \mu(\tilde{q}_k)\text{,}
\end{equation}
the dipole function corresponding to the normal mode coordinates of the system. For the centroid mode ($k=0$), $\omega_k = 0$, meaning that this integral will have no effect on the centroid properties of the system. In addition, for the case of $n = 1$ - the classical system - $g(\vc{q}) = 1$, thus the classical partition function will be unaffected by the presence of an optical cavity, meaning that classical equilibrium constants will be unchanged by vibrational strong coupling.
\\
\indent
Appendix~\ref{app:1-} shows various attempts to transform $g(\vc{q})$ into the bead representations of the ring polymer - which would maybe construction an effective Hamiltonian with the cavity `integrated out'. By then taking the limit of beads to infinity, one could see if the extra term would remain.
\\
\\
With the above information, the partition function of a harmonic oscillator with a linear dipole ($\mu(q) = q$) could be analytically found, giving some idea to the magnitude of cavity influence on partition function. For this system,
\begin{equation}
    V_{\rm H.O.}(q) = \frac{1}{2}\lambda^2q^2
\end{equation}
so the $n$-bead partition function inside a cavity,
\begin{equation}
    Q_{\rm H.O.}^{\rm cav} = \left(\frac{1}{\hbar}\right)^{2n}\!\int\!d\vc{q} \: g(\vc{q}) e^{-\beta_n \sum\limits_{j=1}^{n}\left(\frac{1}{2}\lambda^2q_j^2
+ \frac{1}{2}\omega_n^2(q_j - q_{j+1})^2 \right)} \text{.}
\end{equation}
Which can be transformed into the normal mode representation of the ring polymer to give,
\begin{equation}
    Q_{\rm H.O.}^{\rm cav} = \left(\frac{1}{\hbar}\right)^{2n}\:\:\prod_{k=0}^{n-1}\left[\left(\frac{2\pi(\omega_k^2 +\omega_c^2)}{\beta_n}\right)^{\frac{1}{2}}\!\int\!dq_k e^{-\beta_n \left(\frac{1}{2}\left(\lambda^2
+ \omega_k^2\right)\tilde{q}_k^2 - \frac{C^2\tilde{q}_k^2\omega_c^2}{2}\left(\frac{\omega_k^2}{\omega_k^2 +\omega_c^2}\right) \right)}\right] \text{.}
\end{equation}
All terms can be grouped to give
\begin{equation}
    Q_{\rm H.O.}^{\rm cav} = \left(\frac{1}{\hbar}\right)^{2n}\:\:\prod_{k=0}^{n-1}\left[\left(\frac{2\pi(\omega_k^2 +\omega_c^2)}{\beta_n}\right)^{\frac{1}{2}}\!\int\!dq_k e^{-\beta_n \frac{1}{2}\Omega_k^2\tilde{q}_k^2 }\right] \text{,}
\end{equation}
where - having inserted the definition of $C$ -
\begin{equation}
\Omega_k^2 = \lambda^2
+ \omega_k^2 - \frac{\hbar}{\epsilon_0V}\left(\frac{\omega_k^2}{\omega_k^2 +\omega_c^2}\right)
\end{equation}
The ratio of $n$-bead partition functions inside and outside cavity therefore is the ratio of the product of Gaussians, many factors of which cancel
\begin{equation}
    \frac{Q_{\rm H.O.}^{\rm cav}}{Q_{\rm H.O.}} = \prod_{k=0}^{n-1}\left(\frac{\lambda^2
+ \omega_k^2 - \frac{\hbar}{\epsilon_0V}\left(\frac{\omega_k^2}{\omega_k^2 +\omega_c^2}\right)}{\lambda^2
+ \omega_k^2}\right) ^{-\frac{1}{2}} \text{.}
\end{equation}
% The same method can be followed for $N$ harmonic oscillators coupled to an optical cavity,
% \begin{equation}
%     \hat H_{\rm N} = \sum _{m=1}^{N}\left(\frac{\hat p_m^2}{2} + \frac{1}{2}\lambda^2\hat q_m^2\right) + \frac{\hat p_c}{2} 
%     + \omega_c^2(\hat q_c + C\sum_{m=1}^N\hat q_m )^2
% \end{equation}
% which via a normal modes transform, noting that $[\tilde p_m,\tilde q_n] \propto \delta_{mn}$
% \begin{equation}
%     \hat{H}_{\rm N} = \sum _{k=1}^{N-1}\hat H_{\rm mol}(\tilde{p}_k,\tilde{q}_k) + \hat H_{\rm cav}(\tilde{p}_0,\tilde{q}_0,\tilde{p}_c,\tilde{q}_c) \text{,}
% \end{equation}
% Where $\hat H_{\rm mol}$ is the Hamiltonian of an uncoupled oscillator, and 
% \begin{equation}
%     \hat H_{\rm cav}(\hat p,\hat q,\hat p_c,\hat q_c) = \frac{\hat p^2}{2} + \frac{1}{2}\lambda^2\hat q^2 + \frac{\hat p_c^2}{2} + \frac{1}{2}\omega_c^2(\hat q_c + \sqrt{N}C\hat q)^2\text{.}
% \end{equation}
% As this is now the same Hamiltonian as before, but just with $N - 1$ uncoupled harmonic oscillators, the ratio of partition functions \textbf{per molecule} - for a system of constant Rabi splitting in which $C \leftarrow C/\sqrt{N}$ - will be the same;
% \begin{equation}
%     \frac{Q_{\rm N H.O.}^{\rm cav}}{Q_{\rm N H.O.}} = \prod_{k=0}^{n-1}\left(\frac{\lambda^2
% + \omega_k^2 - \frac{\hbar}{\epsilon_0V}\left(\frac{\omega_k^2}{\omega_k^2 +\omega_c^2}\right)}{\lambda^2
% + \omega_k^2}\right) ^{-\frac{N}{2}} \text{.}
% \end{equation}

==> EXTRA/ROC/ROC.tex <==
\chapter{Reactions Outside Cavity} 

\minitoc

\section{Reactions outside of Cavity}\label{sec: ROC}
This section will introduce the Topaler-Makri model, set up the system-bath model and then will evaluate the reliability of the tools 
\subsection{The Topaler-Makri Model}\label{subsec:TMM}
The model used throughout this thesis is a uni-molecular reaction occurring in double quartic symmetric well\cite{Topaler1994}. Under the Microcannonical Ensemble (NVE) the Classical, mass scaled Hamiltonian for this system is,
\begin{equation}
    H = \frac{p^{2}}{2} + V(q)
\end{equation}
where
\begin{equation}
    V(q) = - \frac{\omega_{b}^2}{2}q^{2}
    + \frac{\omega_{b}^2}{16 E^{\ddagger}}q^{4}
\end{equation}
In real systems though, there is exchange of heat with surroundings such that the Temperature (which is proportional to $\left<E\right>$) is constant, but the Energy of the system itself fluctuates randomly about the mean. For this to be in effect the Caldera-Leggett \cite{Caldeira1985} System-Bath Model will be used.
\subsection{The System-Bath Model}
Commonly used for simulating condensed phase environments is the System Bath Model. The Hamiltonian gains $m$ extra DOF per Degree of Freedom.
\begin{equation}
    H(p,q,\textbf{P},\textbf{Q}) = \frac{p^2}{2} + V(q) + 
    \sum_{i=1}^{m}
    \frac{P_{i}^2}{2} + 
    \frac{1}{2}\omega_{i}^{2}\left(Q_{i} + \frac{c_{i}}{\omega_{i}^{2}}q\right)^{2} 
\end{equation}
The Bath in question has $m$ modes corresponding to disretized spectral density function;
\begin{equation}
    J_{m}(\omega) = \frac{\pi}{2} \sum_{i=1}^{m} 
    \frac{c_{i}^{2}}{\omega_{i}}\delta(\omega-\omega_i)
\end{equation}
The spectral density used by Topaler and Makri is and Ohmic Bath of reorganization energy $\eta$ with an exponential cutoff $\omega_c$, such that;
\begin{equation}
    J_{\infty}(\omega) = \eta \omega e ^{\omega/\omega_c}
\end{equation}
The discretisation scheme, to assign $c_i$ and $\omega_i$ for a given $m$ is also taken form this paper and is;
\begin{equation}
    \omega_{i} = -\omega_{c}\ln\left(\frac{i - 3/2}{m}\right)
    \:\:\:\:\:\:\:\:\:\:\:
    c_{i} = \omega_{i}\left(\frac{2\eta\omega_c}{m\pi}\right)^{\frac{1}{2}}
    \:\:\:
\end{equation}
With this in place, only minor adjustments are needed to simulate the system with the methods introduced in Tools section.\newline
For TST, these extra terms can be added to the Hamiltonian, to alow thermal fluctioations to be taken into account. As all terms remain at most quadratic in $q$ or $Q$, the hessian can be written down. This, once diagonalized allows the hamiltonian to be written down in other coordinates $(\Tilde{q},\Tilde{p})$ of form described in \eqref{eqn:HarmonicHamiltonian}
\subsection{Results}
To test our tools. I will now compare Kramer's Turnover as generated by Makri et al \cite{Topaler1994}l. for the exact Quantum Mechanical and Classical rates of a reaction occurring in the well as defined in \ref{subsec:TMM}. 
\newline\newline
Firstly, the QM and Classical Transition-State Theory estimates of the rate;
\begin{figure}
\centering
\includegraphics{text/ROC/Fig2.png}
\caption{Comparison of Transition State Theory and Exact Rate data \cite{Craig2005}}
\label{fig:fig2}
\end{figure}
As shown, the TST estimate converges to the exact QM and Classical results as $\gamma \rightarrow \infty$, corresponding to a system in which no recrossing is present. \newline \indent
It should be stressed that this TST approximation is NOT the uncoupled TST assumption, but is instead the TST approximation of a system coupled to a bath. This means that on a SINGLE PASS of the transition state, the dynamical corrections WILL be included, but still no recrossing of the transition state will be shown.
\newline \newline
Secondly, RPMD. As 1 Bead is simply the classical Hamiltonian, this should correspond to the exact classical results. As the number of beads is increased, the results should converge to the exact QuantUm Mechanical results. \textbf{RE-RUN THESE}
\begin{figure}
\centering
\includegraphics{text/ROC/Fig3.png}
\caption{Comparison of RPMD and Exact Rate data \cite{Craig2005}}
\label{fig:fig3}
\end{figure}
As mensioned in the tools section, RPMD can capture rates in all regions as, for the Real-Time Quantum Coherences are washed-out in macroscopic systems, and the theory still includes the important effects of Zero-Point Energy and Tunneling \cite{Lawrence2019}.
\newline\newline
This implies that when simulating Polariton Chemistry in the Energy-Diffusion region, only exact rate theory (RPMD and Classical) will be sufficient. For the Spacial-Diffusion regime however, both RPMD and TST \textbf{may} be able to capture these effects.



==> EXTRA/RateTheory1.tex <==
\chapter{\label{RateTheory}Rate Theory} 
why what whats missing

\minitoc


\section{Tools}\label{sec: tools}
This section will offer a derivation of all of the tools used to investigate Polariton chemistry throughout the thesis.
The exact classical and quantum rate can only be found using exact quantum and classical rate theory, but these simulations take lots of time. Transition State Theory coupled with the introduction of time-dependent transmission coeficient , $\kappa(t)$

\subsection{RPMD Rate Theory}

RPMD is a useful tool for simulations of Quantum systems on the large scale. It captures both Zero-Point energy and Tunneling over a reaction barrier. It is exact at $t=0$ but fails to capture any real-time Quantum Coherences such as interference. For macroscopic systems this is not an issue as these effects tend to be 'washed out' due to the large number of particles.

\subsubsection{A Derivation of Ring Polymer Molecular Dynamics (RPMD)}
Here is a derivation of RPMD following the same logic as \cite{Parrinello1984}. The assumed knowledge is as follows. Integrals are over all space unless otherwise specified, also $p$ and $q$ correspond to momenta and position coordinates respectively. These coordinates have the dimensions of the entire system of interest, but here we will stick to 1D (multidimensional generalization is as easy as just changing $q$ and $p$ to vectors of length equal to the dimension of the system); 
\[
\begin{split}
    tr\left[ \hat{O}\right] \equiv \int dq \bra{q}\hat{O}\ket{q} 
    \: \: \: \: \: & \: \: \: \: \: 
    \bra{q}\ket{p} = \sqrt{\frac{1}{2\pi\hbar}}e^{i\hat{p}\hat{q}/\hbar}
    \\
    \hat{1} = \int dp \ket{p}\bra{p}
    \: \: \: \: \:& \: \: \: \: \: 
    \hat{1} = \int dq \ket{q}\bra{q}
\end{split}
\]

\noindent The derivation starts with the definition of the partition function of a system. This is the trace - in the position representation - of the boltzman operator;
\begin{equation}
    Q = tr\left[ e ^{-\beta \hat{H}}\right] \equiv 
    \int dq \bra{q} e ^{-\beta \hat{H}} \ket{q}
\end{equation}
Let us define \begin{math}\beta_{n} = \frac{\beta}{n} \equiv \frac{1}{nk_{B}T}\end{math}. This allows us to factorize the above exponential into \begin{math} n \end{math} terms as such;

\begin{equation}
    Q = \int dq \bra{q}\left(e^{-\beta_{n}\hat{H}}\right)   \left(e^{-\beta_{n}\hat{H}}\right) ... \ket{q}
\end{equation}
\noindent Now, let us insert the identity in between each exponential ($n-1$ times). Each identity corresponds to integration over a different dummy variable, thus the integration must be done $n$ times from $dq_1$ (corresponding to the first $dq$ in the trace above) to $dq_n$ where each integration is independent.

\begin{equation}
    = \int dq_1 ... dq_n \bra{q_1} e^{-\beta_{n}\hat{H}}\ket{q_2}\bra{q_2}   e^{-\beta_{n}\hat{H}}\ket{q_3} ... 
    \bra{q_n}e^{-\beta_{n}\hat{H}}\ket{q_1}
\end{equation}
\noindent This integral now consists of $n$ similar terms of form $\bra{q_{j}}\hat{O}\ket{q_{j+1}}$, with the index modded by $n$ (such that $q_{n+1}\equiv q_{1}$). Looking at one of these terms, by considering the second order Taylor expansion of $\hat{H}$;

\begin{equation}
    \bra{q_j}e^{-\beta_{n}\hat{H}}\ket{q_{j+1}} =
    \bra{q_j}e^{-\frac{\beta_{n}\hat{V}}{2}}e^{-\beta_{n}\hat{T}}e^{-\frac{\beta_{n}\hat{V}}{2}}\ket{q_{j+1}} + o(1/n^3)
\end{equation}
\noindent The potential energies can now be evaluated, on 'either side' (as $\hat{V}$ is hermitian), followed by the insertion of the identity, and integration over $dp$

\begin{equation}
\begin{split}
     \bra{q_j}e^{-\frac{\beta_{n}\hat{V}}{2}}&e^{-\beta_{n}\hat{T}}e^{-\frac{\beta_{j}\hat{V}}{2}}\ket{q_{j+1}} =
     e^{-\frac{\beta_{n}V(q_j)}{2}}
     \bra{q_j}e^{-\beta_{n}\hat{T}}\ket{q_{j+1}}
    e^{-\frac{\beta_{n}V(q_{j+1})}{2}} 
    \\
   & =  \int dp e^{-\frac{\beta_{n}V(q_j)}{2}}
     \bra{q_j}e^{-\beta_{n}\hat{T}}\ket{p}\bra{p}\ket{q_{j+1}}
    e^{-\frac{\beta_{n}V(q_{j+1})}{2}} 
    \\
      &  =  \int dp e^{-\frac{\beta_{n}V(q_j)}{2}}
     \bra{q_j}\ket{p}
     e^{-\frac{\beta_{n}p^2}{2m}}
     \bra{p}\ket{q_{j+1}}
    e^{-\frac{\beta_{n}V(q_{j+1})}{2}} 
        \\
      &  =  \int dp e^{-\frac{\beta_{n}(V(q_j)+V(q_{j+1})}{2}}
     e^{-\frac{\beta_{n}p^2}{2m}-\frac{-ip(q_{j}-q_{j+1})}{\hbar} }
     \\
      &  =  \frac{1}{2\pi\hbar}\sqrt{\frac{2\pi m}{\beta_n}} 
      e^{-\beta_n \left[ \frac{m\omega_n^{2}(q_j - q_{j+1})^2}{2}
      +\frac{V(q_j)}{2}
      +\frac{V(q_{j+1})}{2}\right]}
\end{split}  
\end{equation}
The new parameter $\omega_n$ is equal to $\frac{1}{\beta_n \hbar}$. By now noticing that the pre-factor $\sqrt{\frac{2\pi m}{\beta_n}} $ is of form $\sqrt{\frac{\pi}{\alpha}}$ one can re-introduce the integral over momenta. This is the key step that allows sampling of system using Molecular Dynamics (MD). Therefore;
\begin{equation}
    \bra{q_j}e^{-\beta_{n}\hat{H}}\ket{q_{j+1}} =
\frac{1}{2\pi\hbar}\int dp e^{-\beta_n \left[\frac{p^2}{2m} + \frac{m\omega_n^{2}(q_j -       q_{j+1})^2}{2}
      +\frac{V(q_j)}{2}
      +\frac{V(q_{j+1})}{2}\right]} + o(1/n^3)
\end{equation}
This can now be re-inserted into (2.3) with each integral over $dp$ getting their own index just as in the step proceeding (2.2). Again, all sums and products are cyclical such that  $q_{n+1} \equiv q_{1}$ . Also, the overall error is now of order $1/n^2$ as the approximation of (2.4) is made $n$ times \cite{Craig2005}.
\begin{equation}
\begin{split}
    Q =&
\left(\frac{1}{2\pi\hbar}\right)^n
\int dp_1...dp_n\int dq_1...dq_n
  \prod_{j=1}^{n}
e^{-\beta_n \left[\frac{p_j^2}{2m} + \frac{m\omega_n^{2}(q_j -       q_{j+1})^2}{2}
      +\frac{V(q_j)}{2}
      +\frac{V(q_{j+1})}{2}\right]} + O(1/n^2)
      \\
      =&
      \left(\frac{1}{2\pi\hbar}\right)^n
\int dp_1...dp_n\int dq_1...dq_n
e^{-\beta_n 
\sum\limits_{j=1}^{n}\left[\frac{p_j^2}{2m} 
      + V(q_j)
      + \frac{m\omega_n^{2}(q_j -       q_{j+1})^2}{2}
      \right]} + O(1/n^2)
\end{split}
\end{equation}
By inspection of (2.7) one can see that the partition function is now that of a classical system of extended phase space \cite{} comprised of $n$ copies of the system corresponding to the classical limit of the initial quantum Hamiltonian, with adjacent copies linked together by harmonic springs;
\begin{equation}
\begin{split}
    H_n(\mathbf{p},\mathbf{q}) = \sum\limits_{j=1}^{n}\left[
    \frac{p_j^2}{2m} + V(q_j)+ \frac{1}{2}m\omega_n^{2}(q_j - q_{j+1})^2\right]
    \\
     classical\:lim\:\hat{H}
     \;\;\;\;\;\;\;adjacent\:spring\:potential\:terms
\end{split}
\end{equation}
The phase-space variables $\bold{p}$ and $\bold{q}$ are now vectors containing entries $p_j$ and $q_j$ respectively. The index $j$ corresponds to each 'bead' on the ring polymer, with $n$ giving the total number of beads As $n \xrightarrow{}\infty$,  the error will tend to zero, but as will be shown in results and literature, as the number of beads approaches $40$ the error becomes vanishingly small \cite{Lawrence2019}.

\subsubsection{Classical Rate Theory}
As RPMD is simply classical mechanics in an extended phase space, the classical limit of the exact quantum mechanical rate constant can be used to generate reaction rates.
The exact QM thermal rate constant for a reaction can be shown to be \cite{Miller1983}

\begin{equation}
    k\left(T \right) = \frac{1}{Q_{r}(T)} \lim_{t\to\infty} \overline{c}_{fs}(t)
\end{equation}
\noindent where the flux-side operator, $\overline{c}_{fs}(t)$ is equal to
\begin{equation}
    \overline{c}_{fs}(t) = tr \left[e^{-\beta\hat{H}/2}\hat{F}e^{-\beta\hat{H}/2}e^{+i\hat{H}t/\hbar}  
    \hat{\theta}e^{-i\hat{H}t/\hbar}\right]
\end{equation}
$\overline{c}_{fs}(t)$ is the correlation between flux through the surface dividing reactants and products at time $0$ and the side of the coordinate of the system relative to the surface at time $t$.$\:Q_{r}(T)$ is the reactant partition function per unit length. This is not a transition state-based argurment though as the infinite time limit of$\;\overline{c}_{fs}(t)$ is taken to allow recrossing of the dividing surface.\newline
\indent The classical limit of the rate constant is similarly;

\begin{equation}
     k^{cl}\left(T \right) = \frac{1}{Q_{r}(T)} \lim_{t\to\infty} c^{cl}_{fs}(t)
\end{equation}\noindent
Also the trace in the flux-side correlation function becomes instead a phase-space average, with $q^\ddagger$ corresponding to the value of reaction coordinate at the dividing surface;
\begin{equation}
    c_{fs}^{cl}(t) = \frac{1}{2\pi\hbar} \int dp_{0}\int dq_{0} e^{-\beta H(p_{0},q_{0})}\delta(q_{0}-q^{\ddagger})
    \frac{p_{0}}{m} \theta(q_{t}-q^{\ddagger})
\end{equation}\noindent
Here $\:\theta(x)$ is a Heaviside step function and $\delta(x)$ a Kronecker delta;
\begin{equation}
    \theta(x)
    \begin{cases}
        0 & \text{if } x > 0\\
        1/2 & \text{if } x = 0\\
        1 & \text{if } x > 0
    \end{cases}
    \:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:
        \delta(x)
    \begin{cases}
        0 & \text{if } x > 0\\
        1 & \text{if } x = 0\\
        0 & \text{if } x > 0
    \end{cases}
\end{equation}
This integral can therefore be seen as a sum going over only trajectories starting at the transition state (such that $\delta(q_0 - q^\ddagger) \neq 0$) with terms weighted by its Boltzmann factor and initial momenta; $\frac{p_0}{m}$ . If at time $t$ the trajectory is such that $q_t > q^\ddagger$ , this term remains in the sum. If not, due to the value of $\theta$ being zero, the term is removed. \newline
The limit $c_{fs}^{cl}(t\xrightarrow{}0^+)$ can be shown \cite{} to equal the Transition State Theory rate, as there is no possibility of barrier recrossing. To allow TST to be used, the time-dependent transmission coeficcient, $\kappa(t)$ is introduced.
\newline
The extension of this to RPMD is simply via re-definition of the flux and side operators to allow them to act on the extra-dimensional space.
\subsubsection{Applying this to RPMD}
The RPMD flux-side correlation function is as such \cite{} [cite MOOC HERE];
\begin{equation}
    c_{fs}^{RPMD}(t) = \left(\frac{1}{2\pi\hbar}\right)^{n}
    \int \textbf{dp}_0 \int \textbf{dq}_0
    e^{-\beta_n H_n{(\textbf{p}_0,\textbf{q}_0)}}
    \Dot{\theta}[s(\textbf{q}_0)]
    \theta[s(\textbf{q}_t)]
\end{equation}
The dividing surface between reactants and products is defined at $s(\textbf{q})=0$ and $\dot{\theta}$ is simply the time derivitive of $\theta$, having applied the chain rule;
\begin{equation}
    \dot{\theta}[s(\textbf{q})] = \delta[s(\textbf{q})]\sum\limits_{j=1}^{n}
    \frac{\partial s(\textbf{q})}{\partial q_{j}} 
    \frac{p_j}{m}
\end{equation}
The classical Hamiltonian is that of equation (2.8). It can be shown \cite{Lawrence2019} that the rate of reaction is independent of the choice of $s[\textbf{q}]$ but for simplicity, the function chosen is $s(\textbf{q}) = \frac{1}{n} \sum_{j=1}^{n} q_j$ corresponding to the 'center of mass' or \textbf{centroid} of the system. In a quantum mechanical context, this would correspond to the value of $\left<\hat{q}\right>$ \cite{}CHECKME.\newline\newline
With this framework now in place, molecular dynamics (MD) can be used to sample this integral. A large set of initial phase points are generated, with the centroid fixed to the diving surface at $t=0$ (such that $\delta[s(\textbf{q}_0)] \neq 0 \implies$ initial flux is through the dividing surface) then numerically integrating trajectories according to Hamiltons' Equations ;
\begin{equation}
    \frac{dq_j}{dt} = \frac{\partial H_n}{p_j} \:\:\:\:\:\:\:\:
    \frac{dp_j}{dt} = -\frac{\partial H_n}{q_j}
\end{equation}
These are obtained by application of the Euler-Lagrange equation onto phase space coordinates.\textbf{This} is why RPMD is not able to capture real-time quantum coherences, and as such will not be able to capture shallow tunneling as other methods such as HEOM  \cite{Lindoy2022} would be able to. The exact Quantum Lagrangian would be \cite{Hele2015} 
\begin{equation}
    \hat{L}_{QM} = \frac{p}{m} \frac{\partial}{\partial q} -
    \sum_{\lambda = 1,odd}^{\infty} \frac{1}{\lambda !}
    \left(\frac{i\hbar}{2}\right)^{\lambda -1}
    \frac{\partial^{\lambda}V(q)}{\partial q^{\lambda}}
    \frac{\partial^{\lambda}}{\partial p^{\lambda}}
\end{equation}
But instead RPMD uses the classical limit ($\hbar \xrightarrow{ } 0$) of this expression, corresponding to the classical Liouvillian, thus removing all terms of order $\hbar^2$ and above.
\begin{equation}
    L_{cl} = \frac{p}{m} \frac{\partial}{\partial q} -
    \frac{\partial V(q)}{\partial q}
    \frac{\partial}{\partial p}
\label{eqn:LiouCl}
\end{equation}
With this framework, RPMD Rate theory can be used.

\subsection{Transition State Theory}
The Eyring equation \cite{Eyring1935} as applied for a unimolecular reaction, under Transition-State Theory (TST) is a common tool used by the undergraduate chemist. For a unimolecular reaction, the rate constant is as such;
\begin{equation}
 k(T) = \kappa \frac{k_{B}T}{h} \frac{Q^\ddagger}{Q_r} e^{-\frac{E_0^\ddagger}{k_bT}}
\end{equation}
Where $Q^\ddagger$ and $Q_r$ correspond to the partition functions of the transition state and reactants respectively. As usual, the transition state partition function has one vibrational DOF removed, corresponding to movement over the barrier. \newline
$\kappa$ is the transmission coefficient. This constant accounts for recrossing, which is the making assumption of TST that is invalid in the Energy-Diffusion regime.$E_0^\ddagger$ is the barrier height of the reaction, from the bottom of each well (i.e. \textbf{not} including the Zero-Point Energy of the system)\newline \newline
\indent Now depending on how one builds the partition functions, one can either fine Quantum* or Classical TST rates.
\subsubsection{Classical Transition State Theory}
For any system, the partition function for an $N$ dimensional system can be shown \cite{} to be;
\begin{equation}
    Q = \frac{1}{h^N} \int d\textbf{p}\int d\textbf{q}\: e^{-\beta H(\textbf{p},\textbf{q})}
\end{equation}
where $d\textbf{p}$ corresponds to $dp_1dp_2...dp_N$ (equivalently for $d\textbf{q}$), the integrals are over all space and $\beta = \frac{1}{k_{B}T}$. Suppose the (mass-scaled) Hamiltonian can be written in a harmonic form;
\begin{equation}
    H(\textbf{p},\textbf{q}) =\sum\limits_{i=1}^{N}\left( \frac{p_{i}^2}{2} + \frac{1}{2}\lambda^{2}_i q_i^2 \right)
\label{eqn:HarmonicHamiltonian}
\end{equation}
If this is true, the classical partition function is simply a product of $2N$ independent Gaussian integrals,
\begin{equation}
\begin{split}
Q &= \frac{1}{h^N} \prod_{i=1}^{N}\left( \sqrt{\frac{2\pi}{\beta}} \times \sqrt{\frac{2\pi}{\beta\lambda^{2}_i }}\right) \\
&= \prod_{i=1}^{N} \frac{1}{\beta\hbar\lambda_i } 
\end{split}
\end{equation}
The Hamiltonians used (see section XXXX) are not 100\% of that form but if a second order Taylor expansion of $\:V(q)$ is done at the reacants and transition state, all terms in the potential are square order.
This means that that there exists a Normal Mode transformation that transforms all coordinates to match the form of (2.21) via diagonalization of the Hessian, $V"(q)$, which is the matrix of all second order partial derivitives of the potential. \newline \newline
The classical rate constant is therefore calculated as; 
\begin{equation}
    k^{TST}_{cl} = \frac{\kappa}{2\pi} e^{-\frac{E_0^\ddagger}{k_bT}} \prod_i^\ddagger \frac{1}{\lambda_i} 
    \prod_j^r \lambda_j
\end{equation}

\subsubsection{Quantum Transition State Theory}

Let us 'Ring Polymerise' the Hamiltonian of the previous section, such that the (mass-scaled) Hamiltonian for N degrees of freedom and n beads can be written as;
\begin{equation}
    H_n(\textbf{p},\textbf{q}) =\:\:
    \sum_{j=1}^n \sum_{i=1}^N  \:\:\:\:
     \frac{p_{ij}^2}{2} + \frac{1}{2}\lambda^{2}_{i} q_{ij}^2
    + \frac{1}{2}m\omega_n^{2}(q_{ij} - q_{ij+1})^2
 \end{equation}
 Where $q_{ij}$ corresponds to the coordinated of the $i$th positional DOF on the $j$th bead of the ring polymer and analogous for $p_{ij}$. $\lambda$ has no bead index as for every bead the value is the same as the beads are simply copies of each other.\newline 
 \indent It can be shown \cite{Craig2005} that the partition function of an this system is;
 \begin{equation}
     Q_n = \prod_{l=1}^{n} \prod_{k=1}^N
     \left(4\:\sin^2\left(\frac{l\pi}{n}\right) + \left(\frac{\beta\hbar\lambda_k}{n}\right)^2 \right)^{1/2}
 \end{equation}
 The Classical partition function is the $n=1$ form of the above equation, and the Quantum partition function is;
  \begin{equation}
  \begin{split}
     Q_{QM} &= \lim_{n \xrightarrow{}\infty}\left[\prod_{l=1}^{n} \prod_{k=1}^N
     \left(4\:\sin^2\left(\frac{l\pi}{n}\right) + \left(\frac{\beta\hbar\lambda_k}{n}\right)^2 \right)^{1/2}\right]
     \\
     &= \prod_{k=1}^N\frac{1}{2\:\sinh(1/\beta\hbar\lambda_k)}
\end{split}
 \end{equation}
 So what is meant by the 'Quantum' partition function in this context is simply the $n\xrightarrow{}\infty$ limit of the RPMD partition function, thus including Zero Point Energy and Tunneling but, as usual, no real-time quantum coherences.\newline
 \indent The rate constant for the TST limit of an RPMD system therefore is;
 \begin{equation}
    k^{TST}_{QM} = \kappa \frac{2k_B T}{h} e^{-\frac{E_0^\ddagger}{k_bT}} \prod_i^\ddagger \frac{1}{\sinh(1/\beta\hbar\lambda_i)}
    \prod_j^r\sinh(1/\beta\hbar\lambda_j)
\end{equation}
 With this in place TST theory (for a nicely defined Hamiltonian) can be used.
\subsection{Dynamical Corrections to TST: Kramer's Theory}
The underlying assumption of Transition State Theory is that there is no recrossing of the dividing surface. To this end, it can be shown to be the $t\rightarrow0^+$ limit of the rate constant,\cite{Hanggi1990} or the rate constant corresponding to maximum friction (corresponding to all trajectories starting at the dividing surface being so over-damped that no re-crossing is possible).
\newline\newline
TST theory is sufficient only to describe the short time limit of reaction rates. To fix this, add the changes via the time dependent transmission coefficient \cite{Lec2021};
\begin{equation}
    \kappa(t) = \frac{k(t) }{k(0^+)}
\end{equation}
A relatively simple expression for the transmission coefficient can be found in both the high and low friction limits of a simple $1$D transmission problem.\newline \newline
Kramer's Theory is used to approximate the dynamics at the top of the barrier using Diffusion  at the top. It relies on the steady-state approximation and thus will give the $t \rightarrow \infty$ limit of $\kappa$.\newline \newline 
Grote Hynes Theory is used to approximated dynamics such that the reaction occurs so fast the the other degrees of freedom are shown to be Non-Markovian and need to 'catch-up' with them. This is Non-Markovian dynamics and will be captured using a Generalized Langevin Equation.
\subsubsection{Interlude: First Passage Time}
This equation will be used in the next two sections. The derivation of it  is gorgeous and comes from \cite{Zwan2001}.
\newline \newline\indent
Consider a set of variables $\textbf{a}$, governed by a Langevin equation. Let $\textbf{a}(t)$ and $p(\textbf{a},t)$ be the correspond to the position and distribution of position respectively of $\textbf{a}$ at time $t$. The initial position $\textbf{a}_0$ is in some 'volume' $V$ in $a$-space with a boundary $\partial V$. The initial condition for starting any strajectory at $\textbf{a}_0$ is as such;
\begin{equation}
    p(\textbf{a},0)=\delta(\textbf{a}-\textbf{a}_0) 
\end{equation}
The Fokker-Planck operator, $\mathscr{D}$ corresponding to the Langevin dynamics of the system is defined to evolve the probability distribution of $\textbf{a}$ in time such that;
\begin{equation}
    p(\textbf{a},t)=e^{t\mathscr{D}}p(\textbf{a},0)
\end{equation}
The probability of the particle remaining within the volume $V$ at time $t$ thus equals;
\begin{equation}
    S(t,\textbf{a}_0) = \int_{V}d\textbf{a}\:e^{t\mathscr{D}}\delta(\textbf{a}-\textbf{a}_0)
\end{equation}
Therefore the probability of transmission in some small time $dt$ at $t$ is;
\begin{equation}
\begin{split}
 S(t,a_0)-S(t+dt,a_0) &= \rho(t,\textbf{a}_0) dt
 \\
 \therefore \:\:\:
 \rho(t,\textbf{a}_0) &= -\frac{dS(t,\textbf{a}_0)}{dt}
\end{split}
\end{equation}
And the mean first passage time will be the integral of this probability distribution over all time;
\begin{equation}
    \tau(\textbf{a}_0) = \int_0^\infty dt\int_V d\textbf{a} \:e^{t\mathscr{D}}\delta(\textbf{a}-\textbf{a}_0)
\end{equation}
By inserting unity, and taking the adjoint, the integral can be made such that the operator is only operating on unity, thus allowing integration over $d\textbf{a}$. It should be remembered that $(e^{\hat{O}})^{\dagger} = e^{\hat{O^\dagger}}$ and that the adjoint of a real scalar is itself;
\begin{equation}
\begin{split}
\tau(\textbf{a}_0) &= \int_0^\infty dt\int_{-\infty}^{b}d\textbf{a} \:1\:e^{t\mathscr{D}}\delta(\textbf{a}-\textbf{a}_0)
\\
&= \int_0^\infty dt\int_{-\infty}^{b}d\textbf{a} \:\delta(\textbf{a}-\textbf{a}_0)\: e^{t\mathscr{D}^{\dagger}}\:1
\\
&= \int_0^\infty dt\: e^{t\mathscr{D}^{\dagger}}\:1
\end{split}
\end{equation}
Finally, pre-multiplication by $\mathscr{D}^{\dagger}$ allows mean first passage time to be determined by solving a simple inhomogeneous adjoint equation \cite{Zwan2001}
\begin{equation}
\begin{split}
\mathscr{D}^{\dagger}\tau(a_0) &= \mathscr{D}^{\dagger}\int_0^\infty dt\:e^{t\mathscr{D}^{\dagger}}\:1
\\
&= \int_0^\infty dt\frac{d}{dt}\:e^{t\mathscr{D}^{\dagger}}\:1
\\\ \therefore   \:\:\:
\mathscr{D}^{\dagger}\tau(\textbf{a}_0) =& -1 \:\:\: \text{with}\:\:\: \tau(\textbf{a})=0 \:\text{on}\: \partial v
\label{eqn:FRSTPSGTIME}
\end{split}
\end{equation}
\subsubsection{High-Friction Limit}
Consider a particle crossing a barrier in the presence of other degrees of freedom. In the high-friction limit, the problem can be seen as a first passage time calculation \cite{Zwan2001}. The particle will obey the Langevin Equation;
\begin{equation}
    \ddot{q} = -\gamma \Dot{q} - \frac{dV}{dq} + \sqrt{2\gamma k_BT}\eta
    \:\:\:\:\:\: \left<\eta (t)\eta(t')\right> = 2k_BT\gamma\delta(t-t')
\label{eqn:LE}
\end{equation}
In the \textbf{limit of overdamping} the particle's position will vary slowly, but momentum will be quick. For this reason, the evolution of the particle's phase-space distribution can be equivalently represented with the Fokker-Planck Equation corresponding to the $1$-Dimensional Smulochowski Equation. $D$ is the diffusion coefficient, which in this example is given by the Einstein-Smulochowski relation, $D=\frac{k_BT}{\gamma}$ As it will be useful in the next section, let us treat $D$.
\begin{equation}
\begin{split}
\frac{\partial p(q,t)}{\partial t} &=  \frac{\partial}{\partial q} D e^{-\beta V(q)} \frac{\partial}{\partial q} \left(e^{\beta V(q)} p(q,t)\right) 
\\ \therefore \:\:\:
\mathscr{D}&=  \frac{\partial}{\partial q}D e^{-\beta V(q)} \frac{\partial}{\partial q} e^{\beta V(q)}
\\ \therefore \:\:\:
\mathscr{D}^\dagger&= e^{\beta V(q)}\frac{\partial}{\partial q} e^{-\beta V(q)} D\frac{\partial}{\partial q}   
\label{eqn:SE}
\end{split}
\end{equation}
Using equation \eqref{eqn:FRSTPSGTIME}, the mean first passage time of any trajectory following the above Langevin Equations of Motion can be found;
\begin{equation}
\begin{split}
e^{\beta V(q_0)}\frac{\partial}{\partial q_0} e^{-\beta V(q_0)} D\frac{\partial}{\partial q_0} \: \tau(q_0) = -1
\end{split}
\end{equation}
Now, the boundary conditions. The definition of a reactant is such that $q_0\in(-\infty,q^\ddagger)$ which can be modelled as having an absorbative barrier at $q^\ddagger$ and a reflective barrier at $-\infty$, therefore the equation can be solved for $\tau(q_0)$ by integration, taking these limits into account\textbf{LOOK INTO LIMITS -> DIAGRAM?};
\begin{equation}
\begin{split}
 e^{-\beta V(q_0)} D\frac{\partial}{\partial q_0} \: \tau(q_0) &= -
\int_{-\infty}^{q_0} dq' e^{-\beta V(q')}
\\
\tau(q_0) &=  -\int^{q_0}_{q^\ddagger}dq \frac{e^{\beta V(q)}}{D}
\int_{-\infty}^{q} dq' e^{-\beta V(q')}
\\
&=  \int_{q_0}^{q^\ddagger}dq \frac{e^{\beta V(q)}}{D}
\int_{-\infty}^{q} dq' e^{-\beta V(q')}
\label{eqn:IntSE}
\end{split}
\end{equation}
Now to deal with these integrals. By taking a locally harmonic approximation of the potential at the reactants; $V_R(q) \approx  \frac{1}{2}\omega_{r}^{2}(q-q_r)^2$, and at the dividing surface; $V_\ddagger(q) \approx  E_0^\ddagger - \frac{1}{2}\omega_{b}^{2}(q-q^\ddagger)^2$;
\begin{equation}
\begin{split}
\int_{q_0}^{q^\ddagger}dq e^{\beta V(q)}
\int_{-\infty}^{q} dq' e^{-\beta V(q')}
    \approx 
    \int_{q_0}^{q^\ddagger} dq 
    e^{\beta \left(E_0^\ddagger - \frac{1}{2}\omega_{b}^{2}(q-q^\ddagger)^2\right)} 
    \int_{-\infty}^{q}dq' 
     e^{-\beta \left(\frac{1}{2}\omega_{r}^{2}(q'-q_r)^2 \right)}
\end{split}   
\end{equation}
This approximation is justified as each integral is dominated by the contribution centered at the Taylor Expansion as done. \newline
\indent For the left hand integral, the largest contribution to the integral is when $q \rightarrow q^\ddagger$, therefore this lower limit can be extended to $-\infty$ such that the integral is half of a Gaussian centered at $0$\newline
\indent For the right hand integral, the largest contribution to the integral is when $q \rightarrow q_0$. So, provided $q^\ddagger > q_0$ such that there is minimal overlap between Gaussian double integrals, the upper limit can be extended to $\infty$. \textbf{DIAGRAM NEEDED}
\begin{equation}
\begin{split}
    \int_{q_0}^{q^\ddagger} dq& 
    e^{\beta \left(E_0^\ddagger - \frac{1}{2}\omega_{b}^{2}(q-q^\ddagger)^2\right)}
    \int_{-\infty}^{q}dq' 
     e^{-\beta \left(\frac{1}{2}\omega_{r}^{2}(q'-q_r)^2 \right)}
       \\ &\approx 
    \frac{1}{2}\int_{-\infty}^{\infty} dq 
    e^{\beta \left(E_0^\ddagger - \frac{1}{2}\omega_{b}^{2}(q-q^\ddagger)^2\right)} 
    \int_{-\infty}^{\infty}dq' 
     e^{-\beta \left(\frac{1}{2}\omega_{r}^{2}(q'-q_r)^2 \right)}
\\ 
&= \frac{1}{2}  \:
    \sqrt{\frac{2\pi}{\beta\omega_b^2}}\:e^{\beta E_0^\ddagger}\:\sqrt{\frac{2\pi}{\beta\omega_r^2}}
\\ \\
\therefore\:\:  & \tau \approx \frac{1}{2D}\frac{2\pi k_BT}{\omega_r\omega_b}e^{\beta E_0^\ddagger}
\end{split}
\end{equation}
The rate of arrival to the barrier is $1/\tau$. Note that the  As the arrival can be in either directions, the rate of crossing (in one direction) must equal half of this. Therefore, after inserting the Einstein relation;
\begin{equation}
    k_{SD} = \frac{\omega_b \omega_r}{2\pi\gamma} e^{-\beta E_0^\ddagger}
\end{equation}
By recalling that $\nu_b = \frac{\omega_b}{2\pi} = \frac{k_BT}{h}$ (as used in the derivation of the Eyring Equation), in this high friction or \textbf{spatial diffusion limit} the result is proportional to TST, corresponding to a transmission coefficient as;
\begin{equation}
    \kappa_{SD} = \frac{\omega_b}{\gamma}
\end{equation}
In this limit, the transmission coefficient is dominated by the motion over the barrier, hence the reciprocal dependence on the solvent friction. 
\subsubsection{Low-Friction Limit}
 In the low-friction limit, barrier crossing is frequent, with energy being lost to the surroundings slowly. Once a trajectory has lost enough energy to be confined to a single well, it can be said that the reaction has occured. Thus the rate of relaxation to equilibrium can be said to be controlled by the rate of energy diffusion; hence the \textbf{energy diffusion limit} is this place. The derivation for these dynamics has been copied from \cite{Zwan2001} and starts with the Fokker-Plank equation for the phase space distribution function $f(q,p;t)$ corresponding to the Langevin Equation given in \eqref{eqn:LE}
 \begin{equation}
     \frac{\partial }{\partial t}f(p,q;t) = -L_0 f + \gamma k_BT 
     \frac{\partial}{\partial p} f_{eq}
     \frac{\partial}{\partial p} \frac{f}{f_{eq}}
\label{eqn:FP}
 \end{equation}
 where $L_0$ is the Classical Liouville operator just as in \eqref{eqn:LiouCl} and $f_{eq}$ is the equilibrium distribution, given by the unpeturbed Hamiltonian; $H=\frac{p^2}{2m}+V(q)$\newline\indent
 To transform this distribution into Energy coordinates, integration over distribution for all constant values of energy can be done (I THINK THIS IS EQUIVALENT TO A FOURIER TRANSFORM BUT NOT SURE WHAT)
\newline \newline
The transform is as follows. As energy is conserved for an unpeterbed system, $L_0H=0$
\begin{equation}
\begin{split}
\frac{\partial}{\partial t} g(E;t) &= \int dpdq\:\delta(H-E)\:\frac{\partial}{\partial t} f(q,p;t) 
\\
&= \gamma k_BT \int dpdq\:\delta(H-E)\:\frac{\partial}{\partial p} f_{eq}
     \frac{\partial}{\partial p} \frac{f}{f_{eq}}
\label{eqn:FPT}
\end{split}
\end{equation}
The assumption now comes here. As the position and momenta are varying on a much faster timescale than the total energy of each trajectory in this energy diffusion limit, the distribution function of the particle can be approximated  as some function of the Hamiltonian; $f(q,p;t) \rightarrow \phi(H;t)$ and $f_{eq}(q,p) \rightarrow \phi_{eq}(H)$. This function has the constraint such that it leads to the correct energy distribution;
\begin{equation}
\begin{split}
 g(E;t)&=\int dpdq \delta(H-E)\Phi(H;t)
 \\
 &=\Phi(E;t)\int dpdq \delta(H-E)
 \\
\therefore\:\: \phi(E;t) = \frac{g(E;t)}{\Omega(E)} \:\:\: &\text{and likewise, } \:\:\:
\phi_{eq}(E) = \frac{g_{eq}(E)}{\Omega(E)}
\end{split}
\end{equation}
Where $\Omega(E)$ is the microcanonical partition function. So by insertion of this new definition and application of the chain rule;
\begin{equation}
    \phi_{eq}(E)\frac{\partial}{\partial p} \frac{f(q,p;t)}{f_{eq}(x,p)} 
    \approx 
    \frac{g_{eq}(E)}{\Omega(E)} \frac{p}{m}\frac{\partial}{\partial H}\frac{g(H;t)}{g_{eq}(H)}
\label{eqn:aprox2}
\end{equation}
 Insertion of \eqref{eqn:aprox2} into \eqref{eqn:FPT} and following integration by parts over momentum and observing $\frac{\partial}{\partial p}=\frac{\partial}{\partial E}\frac{p}{m}$, allows \eqref{eqn:FPT} to be written in "Smulochowski" form \cite{Zwan2001} with almost the exact same form as \eqref{eqn:SE};
 \begin{equation}
 \frac{\partial g(E;t)}{\partial t} \approx 
 \frac{\partial}{\partial E} 
D(E)g_{eq}(E)
 \frac{\partial}{\partial E} \frac{g(E;t)}{g_{eq}(E)}
 \end{equation}
 where,
 \begin{equation}
\begin{split}
D(E) = \gamma k_BT \frac{\int dpdq \left(\frac{p}{m}\right)^2 \delta(H-E)}{\Omega(E)}
\end{split}
 \end{equation}
 $D(E)$ is the Energy Diffusion constant. By noticing that $\delta(H-E) \equiv \delta(p^2 - 2m(E-V(q)))$, and thus integrating the numerator over $dp$ yields;
 \begin{equation}
D(E) =  \frac{\gamma k_BT}{m} \frac{\int dq \sqrt{2m(E-V(q))}}
{\Omega(E)}
 \end{equation}
 \textbf{ASK ABOUT SQUARE BRACKETS FOR FUNCTIONALS}\newline
 The integral is over all $q$ such that $E>V(q)$, which in fact corresponds to (half) of the integral of $p(q)$ around a complete cycle of $q$. This is the action; $I(E)$ \cite{Zwan2001} \newline \newline
 *Finally* , we can write down $\tau(E)$, just as in \eqref{eqn:IntSE}, as
 \begin{equation}
     \tau(E_0)=  \int_{E_0}^{E^\ddagger_0}dE \frac{1}{g_{eq}(E)D(E)}
\int_{0}^{E} dE' g_{eq}(E')
 \end{equation}
 Substituting the expressions for $g_{eq}$ and $D(E)$ yields,
 \begin{equation}
     \tau(E_0) = \frac{2m}{\gamma k_BT}
     \int_{E_0}^{E^\ddagger_0}dE
     \frac{e^{\beta E}}{I(E)}
\int_{0}^{E} dE' 
\Omega(E')e^{-\beta E'}
\label{eqn:tauintegral}
 \end{equation}
 At low temperatures, the Mean First Passage Time can be approximated from \eqref{eqn:tauintegral} as;
 \begin{equation}
\begin{split}
 \tau &\approx \frac{2\pi m k_BT}{\gamma}\frac{1}{\omega_r I(E_0^\ddagger)}e^{\beta E_0^\ddagger}
 \\
 \therefore \:\:\: k_{ED} &\approx \frac{\gamma \omega_r I(E_0^\ddagger)}{4\pi m k_BT} e^{-\beta E_0^\ddagger}
 \\
  \therefore \:\:\: \kappa_{ED} &\approx \frac{\gamma \omega_r I(E_0^\ddagger)}{2 m \omega_bk_BT} 
\end{split}
 \end{equation}
 As shown above, $\kappa_{ED} \sim \gamma$ showing that a completely different friction - reaction rate dependence than for high friction.
 \subsubsection{Putting these limits together}
 As shown in these previous sections, $\kappa_{SD}\sim\ \frac{1}{\gamma}$ and $\kappa_{ED}\sim\gamma$. By using Kramer's Interpolation Formula \cite{Kramers1940} these limits can be interpolated to show Kramer's Turnover.
 \begin{equation}
     \frac{1}{\kappa} = \frac{1}{\kappa_{SD}} + \frac{1}{\kappa_{ED}}
 \end{equation}
 When these limits 
 \begin{figure}[H]
\centering
\includegraphics{text/Tools/Fig1.png}
\caption{Connection of the Spacial and Energy Diffusion limits}
\label{fig:fig1}
\end{figure}
As shown in \(\ref{fig:fig1}\) There is some optimum friction where the rate of reaction is maximized. Throughout this thesis there will be graphs that look very similiar to this, and the explanations will follow the same logic. \newline\newline
In this section for dynamical corrections, it was assumed that the friction experienced by any trajectory $\gamma$, was a constant in the equations of motion (see \eqref{eqn:LE} for example). This of course is not true.
\subsection{Grote Hynes Theory}
As proven in \cite{Pollak1986} the Grote-Hynes estimation of the reaction rate is simply the infinite bath mode transition state theory, which will give the reaction rate for a system with no recrossing, but correcting for solvent-induced rotation of the reaction coordinate.\newline\newline
As shown in \cite{Lindoy2022} the recrossing factor can be added to the GH estimate of the reaction rate to allow the rate to be approximated in the Energy-Diffusion regime./

==> EXTRA/anotherproof.tex <==
The equilibrium constant of a reaction can be calculated by the ratio of concentrations of reactants raised to their stoichiometric coefficients. For a quantum system comprised of $N$ equilibria, the total concentration of A 
\begin{equation}
    [{\rm A}] = \frac{\Tr{e^{-\beta \hat H_{\rm tot}}\sum\limits_{i=1}^N \hat \theta_{\text{A}i}}}{\Tr{e^{-\beta \hat H_{\rm tot}}}} \text{,}
\end{equation}
where 
\begin{equation}
\hat \theta_{\text{A}i} = \theta_{\rm A}(\hat q_i) \text{,}
\end{equation}
the projection of the reaction coordinate onto the reactants side. An analogous expression exists for [B], hence the rate constant for this unimolecular equilibirum,
\begin{equation}
    K = \frac{\Tr{e^{-\beta \hat H_{\rm tot}}\sum\limits_{i=1}^N \hat \theta_{\text{B}i}}}{\Tr{e^{-\beta \hat H_{\rm tot}}\sum\limits_{i=1}^N \hat \theta_{\text{A}i}}} \text{.}
\end{equation}
Let us now consider the denominator in more detail. All derivations done here are analogous for the numerator, with the opposite numbering scheme. There are $N+1$ different possibilities for sum of $\theta_{\text{A}i}$, which we will call $S_{\rm A}$. Each sum corresponds to a different region of phase space (the space of all possible combination of $N$ variables that are either A or B)
\begin{center}
\begin{tabular}{c c c } 
 $S_{\rm A}= 0$ & $[N\times{\rm B}]$ & $1 \text{ possible combination}$  \\ [0.5ex] 
 $S_{\rm A} = 1$ & $[{\rm A},(N-1)\times{\rm B}]$ & $N \text{ possible combinations}$ \\ 
  $\vdots$ & $\vdots$ & $\vdots$ \\
  $S_{\rm A} = n$ & $[n\times{\rm A},(N-n)\times{\rm B}]$ & ${N \choose n} \text{ possible combinations}$
\end{tabular}
\end{center}
Therefore by summing over all possibilities the trace can be written as
\begin{equation}
    \Tr{e^{-\beta \hat H_{\rm tot}}\sum\limits_{i=1}^N \hat \theta_{\text{A}i}} = \sum_{n=0}^{N}{N \choose n}
    n\Tr{e^{-\beta \hat H_{n}}} \text{,}
\end{equation}
where $\hat H_{n}$ is the Hamiltonian corresponding to a system of $N$ reaction coordinates, $n$ of which are on side A and $N-n$ of which are on side B. By taking a second order Taylor expansion about the equilibrium potentials of A and B, $V_{\rm A}$ and $V_{\rm B}$. The potential of this hamiltonian, inside of an optical cavity
\begin{equation}
\begin{split}
    \hat{V}_n \simeq nV_{\rm A} + \frac{1}{2}\omega_{\rm A}^2\sum_{i=1}^n  \hat q_{i}^2
    +
    (N&-n)V_{\rm B} + \frac{1}{2}\omega_{\rm B}^2\sum_{j=n+1}^N \!\hat q_{j}^2
\\
+&
\frac{1}{2}\omega_{\rm c}^2\left(\hat q_{\rm c} + g_A\sum_{i=1}^n \hat q_{i} + g_B\sum_{j=n+1}^N \!\hat q_{j}\right)^2 \text{.}
\end{split}
\end{equation}
Now let us rotate into the `Dark'/`Bright' modes of coordinates confined in well A and B. For those in A,
\begin{equation}
     \hat{q}_{\text{A}k} = \frac{1}{\sqrt{n}}\sum_{i=1}^n e^{\frac{2\pi \text{i}}{n}ki}\hat q_i \quad k=0,1,2\:...\:n\!-\!1 \text{.}
\end{equation}
Those in B,
\begin{equation}
     \hat{q}_{\text{B}k} = \frac{1}{\sqrt{N-n}}\sum_{j=1}^{N-n} e^{\frac{2\pi \text{i}}{n}kj}\hat q_{j+n} \quad k=0,1,2\:...\:N\!-\!n\!-\!1 \text{.}
\end{equation}
For both, the $k=0$ corresponds to the totally symmetric linear combination or coordinates, which is commonly known as the `Bright State' due to the fact this is the only linear combination that interacts with the optical cavity. As this is a unitary transformation, the inner product is conserved, such that the potential can be written in the new coordinates as
\begin{equation}
\begin{split}
    \hat{V} \simeq nV_{\rm A} + \frac{1}{2}\omega_{\rm A}^2\sum_{k=0}^{n-1}  \hat q_{\text{A}k}^2
    +
    (N&-n)V_{\rm B} + \frac{1}{2}\omega_{\rm B}^2\sum_{l=0}^{N\!-\!n\!-\!1} \!\hat q_{\text{B}l}^2
\\
+&
\frac{1}{2}\omega_{\rm c}^2\left(\hat q_{\rm c} + g_A\sqrt{n}\: \hat q_{\text{A}0} + g_B\sqrt{N\!-\!n}\:\hat q_{\text{B}0}\right)^2 \text{,}
\end{split}
\end{equation}
which now factors into
\begin{equation}
\begin{split}
    \hat{V} \simeq \sum_{k=1}^{n-1} \hat V_{\rm A}(\hat q_{\text{A}k}) + \sum_{k=1}^{N\!-\!n\!-\!1} \hat V_{\rm B}(\hat q_{\text{B}l})
    + \hat{V}^{\rm bright}_n(\hat q_{\text{A}0},\hat q_{\text{B}0},\hat q_{\rm c}) \text{,}
\end{split}
\end{equation}
where $V_{\rm A}$ and $V_{\rm B}$ are the harmonic potentials for A and B with no cavity present, and 
\begin{equation}
\begin{split}
    \hat{V}^{\rm bright}_n =  V_{\rm A} + \frac{1}{2}\omega_{\rm A}^2 \hat q_{\text{A}0}^2 &+ V_{\rm B} + \frac{1}{2}\omega_{\rm B}^2 \hat q_{\text{B}0}^2 +
\\
 \frac{1}{2}\omega_{\rm c}^2&\left(\hat q_{\rm c} + g_A\sqrt{n}\: \hat q_{\text{A}0} + g_B\sqrt{N\!-\!n}\:\hat q_{\text{B}0}\right)^2 \text{.}
\end{split}
\end{equation}
Let us now combine $\hat{V}^{\rm bright}_n$ back with its momenta such that
\begin{equation}
    \hat{H}^{\rm bright}_n = \frac{\hat p^2_{\text{A}0}}{2} + \frac{\hat p^2_{\text{B}0}}{2} + \frac{\hat p^2_{c}}{2} + \hat{V}^{\rm bright}_n
\end{equation}
Inserting this back into the denominator, tracing over dark states - yielding molecular partition functions $q_{\rm A}$ and $q_{\rm B}$,
\begin{equation}
        \Tr{e^{-\beta \hat H_{\rm tot}}\sum\limits_{i=1}^N \hat \theta_{\text{A}i}} = \sum_{n=0}^{N}{N \choose n}n\:
    q_{\rm A}^{n\!-\!1}q_{\rm B}^{N\!-\!n\!-\!1}\Tr{e^{-\beta  \hat{H}^{\rm bright}_n}}
\end{equation}
The concentration of B can be expressed in an analogous form such that the equilibrium constant, after tracing out the momenta,
\begin{equation}
    K = \frac{\sum\limits_{n=0}^{N}{N \choose n}n\:
    q_{\rm B}^{n\!-\!1}q_{\rm A}^{N\!-\!n\!-\!1}\Tr{e^{-\beta  \hat{V}^{\rm bright}_{n-N}}}}{\sum\limits_{n=0}^{N}{N \choose n}n\:
    q_{\rm A}^{n\!-\!1}q_{\rm B}^{N\!-\!n\!-\!1}\Tr{e^{-\beta  \hat{V}^{\rm bright}_{n}}}} \text{.}
\end{equation}
Now let us introduce $n^\prime = N-n$ and insert into the upper sum,
\begin{equation}
    K = \frac
    {\sum\limits_{n^\prime=0}^{N}{N \choose N-n^\prime}(N-n^\prime)\:
    q_{\rm B}^{N\!-\!n^\prime\!-\!1}q_{\rm A}^{n^\prime\!-\!1}\Tr{e^{-\beta  \hat{V}^{\rm bright}_{n^\prime}}}}
    {\sum\limits_{n=0}^{N}{N \choose n}n\:
    q_{\rm A}^{n\!-\!1}q_{\rm B}^{N\!-\!n\!-\!1}\Tr{e^{-\beta  \hat{V}^{\rm bright}_n}}}\text{.}
\end{equation}
Removing the prime, and cancelling the factors of $q_{\text{A}}$ and $q_{\text{B}}$,
\begin{equation}
    K = \frac{\sum\limits_{n=0}^{N}{N \choose n}n\left(\frac{q_{\rm B}}{q_{\rm A}}\right)^n\Tr{e^{-\beta  \hat{V}^{\rm bright}_n}}}
    {\sum\limits_{n=0}^{N}{N \choose n}(N-n)\left(\frac{q_{\rm A}}{q_{\rm B}}\right)^n\Tr{e^{-\beta  \hat{V}^{\rm bright}_{n}}}} \text{,}
\end{equation}
which now have factors of the cavity-uncoupled equilibrium constant $K_0$ that can be inserted to give,
\begin{equation}
    K = \frac{\sum\limits_{n=0}^{N}{N \choose n}n\:\left(K_0\right)^{n}\Tr{e^{-\beta  \hat{V}^{\rm bright}_n}}}
    {\sum\limits_{n=0}^{N}{N \choose n}(N-n)\:\left(K_0\right)^{-n}\Tr{e^{-\beta  \hat{V}^{\rm bright}_{n}}}} \text{.}
\end{equation}

==> EXTRA/proof.tex <==
It is known (and proven in Appendix~\ref{app:1-}) that any molecular system represented by point charges can be approximated by a set of uncoupled harmonic oscillators, with a linear dipole function. For simplicity, let us consider a 1-Dimensional system of coordinates $\hat p$, $\hat q$ with resonant frequency $\omega$. 
It is known (and proven in Appendix~\ref{app:1-}) that any molecular system represented by point charges can be approximated by a set of uncoupled harmonic oscillators, with a linear dipole function. For simplicity, let us consider a 1-Dimensional system of coordinates $\hat p$, $\hat q$ with resonant frequency $\omega$. 
\begin{equation}
    \hat H_{1}(\hat p,\hat q) = \frac{\hat p^2}{2} +\frac{1}{2}\omega^2\hat q^2 
\end{equation}
Inside of the optical cavity, under mass-scaled coordinates,
\begin{equation}
    \hat H_{\rm tot} = \hat H_{1}(\hat p,\hat q) + \Hat{H}_{\rm cav}(\hat{p}_{\rm c},\hat{q}_{\rm c},\hat \mu)
    \text{,}
\end{equation}
where \begin{equation}
   \Hat{H}_{\rm cav}(\hat{p}_{\rm c},\hat{q}_{\rm c},\hat \mu) =
   \frac{\hat p_{\rm c}^2}{2} +\frac{1}{2}\omega_{\rm c}^2\left(\hat q_{\rm c} + g\hat q\right)^2 \text{.}
\end{equation}
The constant $g$, is the light-matter coupling constant combined with the effective charge and component in polarization direction given to the oscillator. To yield the partition function corresponding to this Hamiltonian, one must diagonalize
\begin{equation}
    \mt{V^{\prime\prime}} = \left(\begin{matrix}
    \omega^2 + g^2\omega_{\rm c}^2 & g\omega_c^2 \\
    g\omega_{\rm c}^2 & \omega_{\rm c}^2
    \end{matrix}\right) \text{,}
\end{equation}
the Hessian matrix corresponding to the Hamiltonian. The eigenvalues of this matrix are 
\begin{equation}
    \Omega^2_\pm = \frac{1}{2}\left(\omega^2 + g^2\omega_{\rm c}^2+\omega_{\rm c}^2\right) \pm \frac{1}{2}\sqrt{\left(\omega^2 + g^2\omega_{\rm c}^2-\omega_{\rm c}^2\right)^2 + 4g^2 \omega_{c}^4} \text{.}
\end{equation}
The partition function can now be expressed in terms of that of uncoupled harmonic oscillators of frequencies $\Omega_\pm$. Firstly for a classical system, using the identity from section~\ref{2:TST},
\begin{equation}
    Q^{\rm cl}_{1} = \frac{1}{\beta \hbar \Omega_+}\frac{1}{\beta \hbar \Omega_-} \text{,}
\end{equation}
which, having inserted $\Omega_\pm$, gives
\begin{equation}
    Q^{\rm cl}_1 = \frac{1}{\beta \hbar \omega_c}\frac{1}{\beta \hbar \omega} \text{,}
\end{equation}
which is simply the classical partition functions of the two uncoupled oscillators. This means that an optical cavity will have no effect on a molecule's classical partition function. For quantum partition functions however,
\begin{equation}
        Q^{\rm qm}_{1} = \frac{1}{2\sinh\left(\beta \hbar \Omega_+/2\right)} \frac{1}{2\sinh\left(\beta \hbar \Omega_-/2\right)} \text{.}
\end{equation}
This expression shows that the partition function \textbf{does} change for a quantum system. The ratio of molecular partition functions gives the equilibrium constant.


The main question, as ever though is will this change in partition function survive in the collective limit?
% \\
% \\
% \indent
% Let us now consider $N$ of these molecular systems at equilibrium, such that the total Hamiltonian inside of a cavity
% \begin{equation}
%     \hat{H}_{\rm tot} = \sum_{i=1}^n\left(\Hat{H}_1(\hat{p}_i,\hat{q}_i)\right) + \Hat{H}_{\rm cav}(\hat{p}_{\rm c},\hat{q}_{\rm c},\hat{\mu}_{\rm tot})\text{,}
% \end{equation}
% where 
% \begin{equation}
%     \hat{\mu}_{\rm tot} = \sum_{i=1}^N \hat \mu(\hat q_i) \text{.}
% \end{equation}
% The Hamiltonian of this system can be expressed in vector form,
% \begin{equation}
%     \hat{H}_{\rm tot} = \frac{1}{2}\omega^2\vc{\hat q}^\top\vc{\hat q} + \frac{1}{2}\vc{\hat p}^\top\vc{\hat p} +  \frac{\hat{p}_{\rm c}^2}{2} + 
% \frac{1}{2}\omega_{\rm c}^2 \left(\hat{q}_{\rm c} + g \sum_{i=1}^N \hat q_i \right)^2 \text{,}
% \end{equation}
% in which 
% \begin{equation}
%     (\vc{\hat q})_i = \hat q_i \quad\text{,}\quad (\vc{\hat p})_i = \hat p_i \text{.}
% \end{equation}
% The coordinates can be transformed into the `dark/bright modes' of the system, such that $\{\hat q\} :\rightarrow\{\hat{\tilde q}\}$ and analogous for $p$.
% \begin{equation}
%      \hat{\tilde q} = \frac{1}{\sqrt{N}}\sum_{l=1}^N e^{\frac{2\pi \text{i}}{N}kl}\hat q_l \quad k=0,1,2\:...\:N-1
% \end{equation}
% the matrix $\mt{K}$ will remain unchanged as it is a diagonal matrix, giving
% \begin{equation}
%     \hat{H}_{\rm tot} = \frac{1}{2}\omega\vc{\hat{\tilde q}}^\top\vc{\hat{\tilde q}} + \frac{1}{2}\vc{\hat{\tilde p}}^\top\vc{\hat{\tilde p}} +  \frac{\hat{p}_{\rm c}^2}{2} + 
% \frac{1}{2}\omega_{\rm c}^2 \left(\hat{q}_{\rm c} + g\sqrt{N} \hat{\tilde q}_0 \right)^2 \text{.}
% \end{equation}
% the Hamiltonian can now be written as
% \begin{equation}
% \hat{H}_{\rm tot} =\left[\sum_{i=1}^{N-1}\left(\Hat{H}_{1}(\hat{\tilde p}_i,\hat{\tilde q}_i)\right)\right] + \left[\Hat{H}_{1}(\hat{\tilde p}_0,\hat{\tilde q}_0)+ \Hat{H}_{\rm cav}\left(\hat{p}_{\rm c},\hat{q}_{\rm c},\hat{\mu}\left(\sqrt{N}\hat{\tilde q}_0\right)\right)\right] \text{.}
% \end{equation}
% Under this new basis, the quantum partition function per molecule
% \begin{equation}
%     Q_N^{\rm qm} = \Tr{e^{-\beta\hat{H}_{\rm tot}}}
% \end{equation}
% can be factorized into
% \begin{equation}
%     Q_N^{\rm qm} = Q_0 \times \prod_{i=1}^{N-1}Q_i
% \end{equation}
% where
% \begin{equation}
%     Q_i = \int d\tilde q_i \bra{\tilde q_i}e^{-\beta\hat{H}_{\rm 1}(\hat{ \tilde p}_i,\hat{\tilde q}_i)}\ket{\tilde q_i} \text{,}
% \end{equation}
% the partition function corresponding to a molecular system \textbf{uncoupled} from an optical cavity and 
% \begin{equation}
%     Q_0 = \int dq_c d\tilde q_0\bra{q_c,\tilde q_0}e^{-\beta\left(\hat{H}_{\rm 1}(\hat{\tilde p}_0,\hat{\tilde q}_0)+\Hat{H}_{\rm cav}(\hat{p}_{\rm c},\hat{q}_{\rm c},\hat{\mu}(\sqrt{N}\hat{\tilde q}_0))\right)}\ket{q_c,\tilde q_0}\text{,}
% \end{equation}
% the single molecule--cavity partition function with $\sqrt{N}$ times the coupling constant. The ratio of \textbf{molecular} partition functions - after cancelling of common factors of uncoupled systems - is therefore 
% \begin{equation}
%     R_{N}^{\rm qm} = \left(\frac{\beta^2\hbar^2\omega\omega_{\rm c}}{4\sinh\left(\beta \hbar \Omega_{N+}/2\right)\sinh\left(\beta \hbar \Omega_{N-}/2\right)}\right)^{\frac{1}{N}} \text{,}
% \end{equation}
% where
% \begin{equation}
%     \Omega^2_{N\pm} = \frac{1}{2}\left(\omega^2 + Ng^2\omega_{\rm c}^2+\omega_{\rm c}^2\right) \pm \frac{1}{2}\sqrt{\left(\omega^2 + Ng^2\omega_{\rm c}^2-\omega_{\rm c}^2\right)^2 + 4Ng^2 \omega_{c}^4} \text{.}
% \end{equation}
% fixed rabi = 
% At large $N$, $R_{N}^{\rm qm}$ tends to $1$ suggesting that an optical cavity will have no effect on a molecular partition function - and therefore any equilibrium constant of a given set of reactants when in a macroscopic system.
